3D Diffuser Actor: Policy Diffusion with 3D Scene Representations

Diffusion policies are conditional diffusion models that learn robot action distributions conditioned on the robot and environment state. They have recently shown to outperform both deterministic and alternative action distribution learning formulations. 3D robot policies use 3D scene feature representations aggregated from a single or multiple camera views using sensed depth. They have shown to generalize better than their 2D counterparts across camera viewpoints. We unify these two lines of work and present 3D Diffuser Actor, a neural policy equipped with a novel 3D denoising transformer that fuses information from the 3D visual scene, a language instruction and proprioception to predict the noise in noised 3D robot pose trajectories. 3D Diffuser Actor sets a new state-of-the-art on RLBench with an absolute performance gain of 18.1% over the current SOTA on a multi-view setup and an absolute gain of 13.1% on a single-view setup. On the CALVIN benchmark, it improves over the current SOTA by a 9% relative increase. It also learns to control a robot manipulator in the real world from a handful of demonstrations. Through thorough comparisons with the current SOTA policies and ablations of our model, we show 3D Diffuser Actor's design choices dramatically outperform 2D representations, regression and classification objectives, absolute attentions, and holistic non-tokenized 3D scene embeddings.

==> 1_abstract_new.tex <==
\begin{abstract}
%We marry  diffusion  policies and 3D scene representations for robot manipulation. 
Diffusion policies are conditional diffusion models that learn robot action distributions  conditioned on the robot and environment state.  They have recently shown to outperform both deterministic and alternative action distribution learning  formulations.  
3D robot policies use 3D scene feature representations aggregated  from a single or multiple camera views using sensed depth. They have shown to  generalize better than their 2D counterparts across camera viewpoints. 
We unify these two lines of work and present \modellong{}, a neural policy  
equipped with a novel 3D   denoising transformer  that fuses information from the  3D visual scene, a language instruction and proprioception %, noised 3D robot pose trajectories, language instructions and proprioception 
to predict the  noise in  noised 3D robot pose trajectories.  %predict the noise
%At each denoising iteration, our model represents end-effector pose estimates as 3D scene tokens and predicts the 3D translation and rotation error for each of them, by featurizing them using 3D relative attention to other 3D visual and language tokens. 
\modellong{} sets a new state-of-the-art on RLBench with an absolute performance gain of 18.1\%  over the current SOTA on a multi-view setup and an absolute gain of 13.1\% on a single-view setup. 
On the CALVIN benchmark, it improves over the current SOTA 
%in the setting of zero-shot unseen scene generalization by being able to successfully 
by a 9\% relative increase. 
It also learns to control a robot manipulator in the real world from a handful of demonstrations. 
Through thorough comparisons with the current SOTA policies and ablations of our model, 
we show \modellong's  design choices dramatically outperform 2D  representations, regression and classification objectives, absolute attentions, and holistic non-tokenized 3D scene embeddings.  
\end{abstract}




==> 2_introduction_new.tex <==
\section{Introduction}
\label{sec:intro}

Many robot manipulation tasks 
are inherently multimodal: at any point during task execution, there may be multiple actions which yield task-optimal behavior. Indeed, human demonstrations often contain diverse ways that a task can be accomplished. 
A natural choice  is then to treat policy learning as a distribution learning problem: instead of representing a policy as a deterministic map $\pi_\theta(x)$,  learn the entire distribution of actions conditioned on the current robot state $p(y|x)$ \cite{DBLP:journals/corr/HoE16,tsurumine2022goalaware,DBLP:journals/corr/HausmanCSSL17,shafiullah2022behavior}. 


Recent works  use diffusion objectives for learning such state-conditioned action distributions for robot manipulation policies from demonstrations \cite{pearce2023imitating,chi2023diffusion,reuss2023goal}. 
They outperform  deterministic or other  alternatives, such as variational autoencoders \cite{IRIS}, mixture of Gaussians \cite{10.1145/1329125.1329407}, combination of classification and regression objectives \cite{shafiullah2022behavior}, or energy-based objectives \cite{DBLP:journals/corr/abs-2109-00137}. %Specifically, they exhibit better action distribution coverage and higher fidelity (less mode hallucination) than alternative formulations \cite{pearce2023imitating}.  
They typically use either low-dimensional (oracle) states \cite{pearce2023imitating} or 2D  images   \cite{chi2023diffusion} as their scene representation. 

\begin{comment}
\input{src/fig_teaser}
\end{comment}

% \begin{figure*}[h!]
%     \centering
%     \begin{adjustbox}{center}
%     \includegraphics[width=1.0\textwidth,keepaspectratio]{figs/teaser.pdf}
%     \end{adjustbox}    
%     \caption{{\textbf \model{}} is a language and vision conditioned action diffusion policy that learns to predict end-effector keyposes and trajectories from demonstrations.  (a) An image encoder  extracts a 2D image feature map from each camera view;  each feature token corresponds to a fixed-size patch in the input image. 
%     (b) We lift  2D feature tokens to 3D using sensed depth.  \rebut{(c) We encode language instructions with a pre-trained language encoder.  (d)} A 3D relative position attention Transformer  takes as input   the 3D scene tokens, an instruction text encoding,  a short history of  end-effector poses and the current noisy estimate of the end-effector future trajectory (or keypose) and outputs the noise in the form of 3D translations and rotations.
%     }
%     \label{fig:overview}
% \end{figure*}

At the same time, 3D robot policies build %bird's eye view (BEV) or 
scene representations by ``lifting" features from perspective views to a  3D  robot workspace based on sensed depth and camera extrinsics  
%such as Transporter Networks  
\cite{zeng2021transporter,huang2024fourier, james2022coarse, shridhar2023perceiver,gervet2023act3d,goyal2023rvt}. 
%They , and  have  shown strong  empirical results %in robot learning from demonstrations
%\cite{shridhar2023perceiver, james2022coarse, goyal2023rvt, gervet2023act3d}. 
They  have shown to 
%Policies that use such 2D-to-BEV or 2D-to-3D scene encodings
generalize better than  2D robot policies across camera viewpoints and  to handle   novel camera viewpoints at test time \cite{gervet2023act3d,goyal2023rvt}. We conjecture this improved performance comes from the fact that the visual scene tokens and the robot's actions interact in a common 3D space, that is robust to camera viewpoints, while in 2D policies the neural network need to learn the 2D-to-3D mapping implicitly. % across views.  
 
 
 %3D robot policies have not yet been combined yet with diffusion objectives. One exception is ChainedDiffuser \cite{xian2023chaineddiffuser}, 
 %which uses a diffusion model that takes as input 3D end-effector keyposes predicted by Act3D \cite{gervet2023act3d} and a 3D representation of the scene to infer end-effector 3D trajectories that link the current end-effector pose to the predicted one. ChainedDiffuser 
 %that uses diffusion models as a drop-in replacement for motion planners, rather than  manipulation policies, since it relies on other learning based policies (\cite{gervet2023act3d}) to supply the target 3D keypose to reach. We compare against ChainedDiffuser in our experiments and show we greatly outperform it.

In this work, we   marry  diffusion  for handling  multimodality in action prediction with 3D scene representations for effective spatial reasoning. We propose \modellong{}, a novel 3D  denoising policy transformer 
that takes as input a tokenized 3D scene representation, a language instruction and a  noised end-effector's  future translation and rotation trajectory, and  predicts the error in translations and rotations for the robot's end-effector. 
The model %achieves translation equivariance in prediction by 
represents both the scene tokens and the end-effector locations in the same 3D space and fuses them with 
%representing the current estimate of the robot's end-effector trajectory as 3D scene tokens and featurizing them jointly with the visual tokens using 
relative-position 3D attentions \cite{shaw2018selfattention,su2021roformer}, which achieves translation equivariance and helps generalization. 
%In this way, the model does not depend

%, as shown in Figure \ref{fig:overview}. 



We test \modellong{} in  learning robot manipulation policies from demonstrations on the simulation benchmarks of RLBench \cite{james2020rlbench} and CALVIN \cite{mees2022calvin}, as well as in the real world. \modellong{} sets a new state-of-the-art on RLBench with a 18.1\% absolute gain on multi-view setups and 13.1\% on single-view setups, outperforming existing 3D policies and 2D diffusion policies. On CALVIN, it outperforms the current SOTA in the setting of zero-shot unseen scene generalization by a 9\% relative gain. We further show \modellong{} can learn multi-task manipulation in the real world across 12 tasks from a handful of real-world demonstrations. 
%Through extensive ablations and comparisons, 
We empirically show that \modellong{} outperforms all existing policy formulations, which either do not use 3D scene representations, or do not use action diffusion.   
We further compare against  ablative versions of our model and show the importance of the 3D relative attentions. % transformer backbone, as well as against version that use  

\textbf{Our contributions:} The main contribution of this work is to combine 3D scene representations and diffusion objectives for learning robot policies from demonstrations. 3D robot policies have not yet been combined  with diffusion objectives. An  exception is ChainedDiffuser \cite{xian2023chaineddiffuser},  that uses diffusion models as a drop-in replacement for motion planners, rather than  manipulation policies, since it relies on other learning-based policies (Act3D \cite{gervet2023act3d}) to supply the target 3D keypose to reach. 
 We compare against ChainedDiffuser in our experiments and show we greatly outperform it. 
 


 \textbf{Concurrent work:} Concurrent to our effort, 3D diffusion policy~\cite{Ze2024DP3} shares a similar goal of combining 3D representations with diffusion objectives for learning manipulation from demonstrations. Though the two works share  the same goal, they have very different  architectures. Unlike \modellong{}, the model of \cite{Ze2024DP3} does not condition on a tokenized 3D scene representation but rather on a holistic  1D embedding pooled from the 3D scene point cloud.  We compare \modellong{} against \cite{Ze2024DP3} in our experiments and show it greatly outperforms it. %This shows the importance of the 3D tokenized and thus spatially disentangled representation using in our model. %jointly reasoning about the scene and robot actions in a disentangled 3D space, where a transformer architecture can relate actions based on the nearest 3D visual tokens. 
 We believe this is because tokenized scene representations, used in \model{}, are robust to scene changes: if a part of the scene changes, only the corresponding subset of  3D scene tokens  is affected. In contrast,  holistic scene embeddings pooled across the scene are always affected by any scene change. Thanks to this spatial disentanglement of the 3D scene tokenization,  \modellong{} generalizes  better. 

%Simulation and real-world robot execution videos, as well as our code and trained checkpoints are publicly available on our website: \url{3d-diffuser-actor.github.io}.

%\HL{In summary, our  contributions are as follows:
%\begin{enumerate}
%\item  Combining 3D scene representations with diffusion objectives for learning robot policies. 
%\item State-of-the-art performance in established benchmarks, much above previous works.
%\end{enumerate}
%}

Our models and code will be publicly available upon publication. Videos of our manipulation results are available at \url{https://sites.google.com/view/3d-diffuser-actor}.

%\url{}. \todo{+++ Is this allowed, to link websites?}
% Simulation and real-world robot execution videos are included as part of our supplementary material. 



==> 3_relatedwork_new.tex <==
\section{Related Work}
\label{sec:work}


 

\noindent \textbf{Learning manipulation policies from demonstrations}
%Though state-to-action mappings are typically multimodal, 
Earlier works on learning from demonstrations train deterministic policies with behavior cloning \cite{Pomerleau-1989-15721,DBLP:journals/corr/BojarskiTDFFGJM16}. 
To better handle action multimodality,  approaches  discretize action dimensions  and use cross entropy losses \cite{semanetlang,shridhar2023perceiver,zeng2021transporter}. 
%However, the number of bins needed to approximate a continuous action space grows exponentially with increasing dimensionality. 
Generative adversarial networks \cite{DBLP:journals/corr/HoE16,tsurumine2022goalaware,NEURIPS2019_c8d3a760}, variational autoencoders \cite{IRIS},   combined Categorical and Gaussian distributions \cite{shafiullah2022behavior,guhur2023instruction,Cui2022FromPT} and Energy-Based Models (EBMs) \cite{DBLP:journals/corr/abs-2109-00137,ta2022conditional,gkanatsios2023energy}  have been used to learn from multimodal demonstrations. 
%Nevertheless, these models tend to be sensitive to hyperparameters, such as the number of clusters used \cite{shafiullah2022behavior}.
%Implicit behaviour cloning  represents distributions over actions by using Energy-Based Models (EBMs) \cite{DBLP:journals/corr/abs-2109-00137,ta2022conditional}. Optimization in EBMs amounts to searching the energy landscape for minimal-energy action, given a state. EBMs are inherently multimodal, since the learned landscape can have more than one minima. 
%EBMs are also composable, which makes them suitable for combining action distributions with additional constraints during inference \cite{gkanatsios2023energy}. 
Diffusion models \cite{sohldickstein2015deep,DDPM} are a powerful class of generative models related to EBMs in that they   model the score of the  distribution, else, the gradient of the energy, as opposed to the energy itself \cite{singh2023revisiting,salimans2021should}. The key idea behind diffusion models is to iteratively transform a simple prior distribution into a target distribution by applying a sequential denoising process. They have been used for modeling state-conditioned action distributions in imitation learning \cite{ryu2023diffusion,urain2023se,pearce2023imitating,wang2022diffusion,reuss2023goal,mishra2023reorientdiff}  from low-dimensional input, as well as from visual sensory input,
and show both better mode coverage and higher fidelity in action prediction than alternatives. 
%They have not been yet combined with 3D scene representations.


\noindent\textbf{Diffusion models in robotics}
Beyond policy representations in imitation learning, diffusion models have been used to model cross-object and object-part arrangements \cite{liu2022structdiffusion,simeonov2023shelving,mishra2023reorientdiff,fang2023dimsam,gkanatsios2023energy}, visual image subgoals \cite{kapelyukh2023dall,dai2023learning,ajay2023hip,black2023zero},  and 
%They have also been used successfully in 
offline reinforcement learning \cite{chen2023offline,yang2024diffusiones,hansen2023idql}. 
%, where they model the state-conditioned action trajectory distribution \cite{hansen2023idql,chen2023offline} or state-action trajectory distribution \cite{janner2022planning, he2023diffusion, Wang2023ColdDO}.
ChainedDiffuser~\cite{xian2023chaineddiffuser}  proposes to replace motion planners, commonly used for  keypose  to keypose linking, with a trajectory diffusion model that conditions on the 3D scene feature cloud and the predicted target 3D keypose to denoise a trajectory from the current to the target keypose. It 
 uses a diffusion model that takes as input 3D end-effector keyposes predicted by Act3D \cite{gervet2023act3d}  and a 3D representation of the scene to infer  robot end-effector  trajectories that link the current end-effector pose to the predicted one. 3D Diffuser Actor instead predicts the next 3D keypose for the robot's end-effector alongside the linking trajectory, which is a much harder task than linking two given keyposes.  %The reason is that their keypose prediction model is deterministic 
 %and  cannot handle  multimodality well. 
 %\model{}  directly predicts future end-effector trajectories in one shot, having a much simpler implementation besides superior performance. 
3D Diffusion Policy~\cite{Ze2024DP3} also  combines 3D scene representations with diffusion objectives but uses 1D point cloud embeddings. We compare against both ChainedDiffuser and 3D Diffusion Policy in our experimental section and show we greatly outperform them.   %Lastly, image diffusion models have  been used for augmenting the conditioning  images input to robot policies to help the latter generalize better \cite{liang2023adaptdiffuser,chen2023genaug,mandi2022cacti}. 


\noindent\textbf{2D and 3D scene representations for robot  manipulation} 
End-to-end image-to-action policy models, such as RT-1~\cite{brohan2022rt}, RT-2~\cite{brohan2023rt2}, GATO~\cite{reed2022generalist}, BC-Z~\cite{jang2022bc}, RT-X~\cite{Padalkar2023OpenXR}, Octo~\cite{octo_2023} and InstructRL~\cite{liu2022instruction} leverage transformer architectures for the direct prediction of 6-DoF end-effector poses from 2D video input. However, this approach comes at the cost of requiring thousands of demonstrations to implicitly model 3D geometry and adapt to variations in the training domains. %Another line of research is centered around Transporter networks \cite{zeng2021transporter,seita2021learning,shridhar2022cliport, gkanatsios2023energy}, demonstrating remarkable few-shot generalization by framing end-effector pose prediction as pixel classification. Nevertheless, these models are usually confined to top-down 2D planar environments with simple pick-and-place primitives. 
3D scene-to-action policies, exemplified by C2F-ARM~\cite{james2022coarse} and PerAct~\cite{shridhar2023perceiver}, involve voxelizing the robot's workspace and learning to identify the 3D voxel containing the next end-effector keypose.   %(Figure~\ref{fig:compare} (b)).  
However, this becomes computationally expensive as resolution requirements increase. Consequently, related approaches resort to either coarse-to-fine voxelization, equivariant networks \cite{huang2024fourier} or efficient attention operations~\cite{jaegle2021perceiver} to mitigate computational costs. 
Act3D \cite{gervet2023act3d} 
%(Figure~\ref{fig:compare} (a)) 
foregoes 3D scene voxelization altogether; it instead computes a 3D action map of  variable spatial resolution by sampling 3D points in the empty workspace and featurizing them using cross-attentions to the  3D physical scene points. Robotic View Transformer (RVT) \cite{goyal2023rvt} re-projects the input RGB-D image to alternative image views, featurizes those and lifts the predictions to 3D to infer 3D locations for the robot's end-effector. 




\model{} builds upon works of Act3D \cite{gervet2023act3d} from 3D policies and upon the works of \cite{urain2023se,chi2023diffusion} from diffusion policies. It uses a tokenized 3D scene  representation, similar to \cite{gervet2023act3d}, but it is a probabilistic model instead of a deterministic one. It does not sample 3D points and does not infer 3D action maps. It uses diffusion objectives instead of  classification or regression objectives used in \cite{gervet2023act3d}. In contrast to \cite{simeonov2023shelving,urain2023se}, it uses 3D scene representations instead of 2D images or low-dimensional states.  
We compare against both 2D diffusion policies and 3D policies in our experiments and show \modellong{} greatly outperforms them. 
%Act3D is a deterministic model, sampling and scoring 3D points in a coarse-to-fine manner to predict 3D locations and regress 3D orientations. \model{} foregoes predicting 3D action maps altogether and considers action prediction as a denoising process conditioned on  images and language instructions, instead of a point classification problem. 
We highlight the differences between our model  and related models in Figure~\ref{fig:compare} in the Appendix, and 
we refer to Figures \ref{fig:detailed_diagram} and \ref{fig:act3d_detailed_diagram} for more architectural details of \model{} and Act3D.%, and to Figure~\ref{fig:compare} for a visual depictions of the differences between our model  and related models.  %on the technical differences between Act3D and \model{}. %Both Act3D and RVT show currently the highest performance on RLBench \cite{james2020rlbench}.
%Our model outperforms Act3D and RVT by a big margin, as we show in the experimental section.

\begin{comment}
\noindent \textbf{Instruction-conditioned policies}
To generate actions based on language instructions, early works~\cite{lynch2020language,mees2022hulc,brohan2022rt} employ a text encoder to map language instructions to latent features,  then they deploy 2D policies that condition on these language latents to predict actions. HULC++ \cite{mees2023grounding} alternates between a free-space policy that reaches subgoals (next object to interact with) and a local policy \cite{mees2022hulc} for low-level interaction. However, these models struggle to infer 3D actions precisely from 2D observations and language instructions and do not generalize to new environments with different texture.  Recent works~\cite{black2023zero,li2023vision,wu2023unleashing} explore the use of large-scale pre-training to boost their performance. SuSIE~\cite{black2023zero} proposes to synthesize visual subgoals using InstructPix2Pix~\cite{brooks2023instructpix2pix}, an instruction-conditioned image generative model pre-trained on a subset of 5 billion images~\cite{schuhmann2022laion}.  Actions are then predicted by a low-level diffusion policy conditioned on both current observations and synthesized visual goals.  RoboFlamingo~\cite{li2023vision} fine-tunes existing vision-language models, pre-trained for solving vision and language tasks, to predict the robot's actions.  GR-1~\cite{wu2023unleashing} pre-trains a GPT-style transformer for video generation on a massive video corpus, then jointly trains the model for predicting robot actions and future observations. We show that \model{} can exceed the performance of these policies thanks to effective use of 3D representations.
\end{comment}

==> 4_method_new.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{src/fig_arch}
% \figArchitecture{htb}


\section{Method}


\label{sec:method}

3D Diffuser Actor is 
trained to imitate  demonstration  trajectories of the form of $\{(\oo_1, \ac_1), (\oo_2, \ac_2), ...\}$, accompanied with a task language instruction $\lang$, similar to previous works \cite{james2022q, shridhar2023perceiver, gervet2023act3d, wu2023unleashing}, where $\oo_t$ stands for the visual observation and $\ac_t$ stands for robot action at timestep $t$. Each observation $\oo_t$ is one or more posed  RGB-D images. %Each trajectory $\tr$ is a sequence of actions $\ac_{t=1:T}$, with $t$ the trajectory timestep and $T$ the temporal horizon. 
Each action $\ac_t$ is an end-effector pose and is decomposed into 3D location, rotation and binary (open/close) state: 
$\ac_t = \{ \ac_t^{\mathrm{\small loc}} \in \mathbb{R}^3, \ac_t^{\mathrm{\small rot}} \in \mathbb{R}^6, \ac_t^{\mathrm{\small open}} \in \{0,1\}\} $. We represent rotations using the  6D rotation representation
of \cite{zhou2020continuity} for all environments in all our experiments, to avoid the discontinuities of the quaternion representation.  We will use the notation $\tr_t=(\ac_{t:t+T}^{\mathrm{\small loc}}, \ac_{t:t+T}^{\mathrm{\small rot}})$ to denote the trajectory of 3D locations and rotations at timestep $t$, of temporal horizon $T$. Our model, at each timestep $t$ predicts a trajectory $\tr_t$ and binary states $\ac_{t:t+T}^{\mathrm{\small open}}$.%, which the robot executes before planing the next trajectory. %Trajectories can have varying lengths $T$.  %trajectories at 
%3D Diffuser Actor 
% \todo{??NIKOS}

%
The architecture of \model{} is shown in Figure~\ref{fig:architecture}. 
It is a conditional diffusion probabilistic model \cite{sohldickstein2015deep,ho2020denoising}  of trajectories given the visual scene and a language instruction; it predicts a whole trajectory $\tr$ at once, non autoregressively, through iterative denoising, by inverting a process that gradually adds noise to a sample $\tr^0$.  % and poses the data-generating process as an
%iterative denoising procedure. 
%This denoising is the reverse of a forward diffusion process 
%that slowly corrupts the structure in data by adding noise. 
%Here, we focus on modelling trajectories $\tr$ of the robot's end effector.
%A diffusion model learns to model a probability distribution $p(\tr)$ by inverting a process that gradually adds noise to a sample $\tr$. 
%For us, $x$ represents a sequence of 3D translations and 3D rotations for the robot's end-effector.  % for a t's future trajectory. 
The diffusion process is associated with a variance schedule $\{\beta^\id \in (0,1)\}_{\id=1}^{\maxid}$, which defines how much noise is added at each diffusion step. The noisy version of sample $\tr^0$ at diffusion step $\id$ can then be written as $\tr^\id = \sqrt{\bar{\alpha}^\id} \tr^0 + \sqrt{1-\bar{\alpha}^\id} \epsilon$, where
$ \epsilon \sim \mathcal{N}(\bzero,\bone)$ 
is a sample from a Gaussian distribution (with the same dimensionality as $\tr^0$), $\alpha^\id = 1- \beta^\id$, and $\bar{\alpha}^\id = \prod_{j=1}^\id \alpha^j$.%\fixme{In \model{}, we exclude binary state $\ac^{\mathrm{\small open}}$ from sample $\tr$, where the model takes input as noised locations $\ac^{\mathrm{\small loc}}$ and rotations $\ac^{\mathrm{\small rot}}$, consists of 3D locations and 3D rotations }


\noindent\textbf{3D Relative  Denoising Transformer} 
\model{} models a learned gradient of the denoising process with a 3D relative transformer 
%The denoising process is modeled by a neural network 
$\hat \epsilon = \epsilon_{\theta}(\tr_t^\id;\id,\oo_t,\lang, \hist_t)$ 
that takes as input the noisy trajectory $\tr_t^\id$ at timestep $t$, diffusion step $\id$, and conditioning information from the language instruction $\lang$, the visual observation $\oo_t$ and proprioception $\hist_t$ of timestep $t$, to predict the noise component $\hat \epsilon$.
At each timestep $t$ and diffusion step $\id$, we convert visual observations $\oo_t$, proprioception $\hist_t$ and noised trajectory estimate $\tr_t^i$ to a set of 3D tokens. Each 3D token is represented by a  latent embedding and  a 3D position. Our model fuses all 3D tokens using relative 3D attentions, and additionally fuses information from the language instruction using normal attentions, since it is meaningless to define 3D coordinates for language tokens. 
Next, we describe how we featurize each piece of input (when not ambiguous, we omit the subscript $t$ for clarity). %We omit timestep $t$ notation for clarity.%, since we refer to a specific timestep. 


\noindent \textbf{3D tokenization} At each diffusion step $\id$, we represent the noisy estimate $\tr^\id$ of the clean trajectory $\tr^0$ as a sequence of 3D trajectory tokens, by mapping each noisy pose $\ac^\id$ of $\tr^\id$,  to a latent embedding vector with a MLP, and a 3D position which comes from the noised 3D translation component $\ac^{loc,\id}$.  
We featurize each image view using a 2D feature extractor  and obtain a corresponding 2D feature map $F \in \mathbb{R}^{H \times W \times c}$, where $c$ is the number of feature channels and $H, W$ the spatial dimensions, using a pre-trained CLIP ResNet50 2D image encoder ~\cite{radford2021learning}. Given the corresponding depth map from that view, we  compute the 3D location $(X,Y,Z)$ for each of the $H \times W$ feature patches by averaging the depth value inside the patch extent.  
We map the pixel coordinate and depth value of a patch to a corresponding 3D coordinate using camera intrinsics and extrinsics and the pinhole camera model. 
This results in a 3D scene token set of cardinality $H \times W$. Each scene token is represented by the corresponding patch feature vector $F_{x,y}$, the feature vector at the corresponding patch coordinate $(x,y)$,  
and a 3D position. If more than one views are available,  we aggregate 3D scene tokens from each, to obtain the final 3D scene token set. %We use a pre-trained CLIP ResNet50 2D image encoder ~\cite{radford2021learning} to encode each RGB image into a 2D feature map.  
The proprioception $\hist$ is also a 3D scene token, with a learnable latent representation and the 3D positional embedding corresponding to the end-effector's current 3D location.  
Lastly, we map the language task instruction to language tokens using a pre-trained CLIP language encoder, following previous works \cite{gervet2023act3d}. 


%This sequence attends to 3D scene tokens and language instruction tokens to predict the noise $\eps^\id$ added to $\tr^0$ at diffusion step $\id$.








Our 3D Relative  Denoising Transformer applies relative self-attentions among all 3D tokens, and cross-attentions to the language tokens. % and all pose tokens using their 3D locations and $\ac_{1:T}^{pos, i}$ respectively.  %To ensure translation invariance in the denoising transformer, 
For the 3D self-attentions, we use the rotary positional embeddings~\cite{su2021roformer} to encode relative positional information in attention layers.  The attention weight between query $q$ and key $k$ is written as: $e_{q, k} \propto \mathbf{x}_q^T \mathbf{M}(\mathbf{p}_q - \mathbf{p}_k) \mathbf{x}_k$, where $\mathbf{x}_q$ / $\mathbf{x}_k$ and $\mathbf{p}_q$ / $\mathbf{p}_k$ denote the features and 3D positions of the query / key, and $\mathbf{M}$ is a matrix function which depends only on the relative positions of the query and key, inspired by recent work in visual correspondence \cite{Li2021LepardLP,Gkanatsios2023AnalogyFormingTF} and 3D manipulation \cite{gervet2023act3d,xian2023chaineddiffuser}. 
We feed the final trajectory tokens to MLPs to predict: (1) the noise $\epsilon^{loc}_\theta(\oo, \lang, \hist,\tr^\id, \id)$ and $\epsilon^{rot}_\theta(\oo, \lang, \hist,\tr^\id, \id)$ added to $\tr^0$'s sequence of 3D translations and 3D rotations, respectively, and (2) the end-effector opening $f_\theta^{\mathrm{\small open}}(\oo, l, c,\tr^\id,i)\in [0,1]^T$. 


\noindent \textbf{Training and inference}
During training, we randomly sample a time step $t$ and a diffusion step $\id$ and add noise $\epsilon = (\epsilon^{\mathrm{\small loc}}, \epsilon^{\mathrm{\small rot}})$ to a ground-truth trajectory $\tr_t^0$.  
%We supervise \model{} using a denoising objective: conditioning on the tuple of $(o, l, c, i)$, our model learns to reconstruct the clean actions by predicting the pose transformation with respect to the current trajectory estimate $\tr^i$. 
We use the $L1$ loss for reconstructing the sequence of 3D locations and 3D rotations. We use binary cross-entropy (BCE) loss to supervise the end-effector opening $f_\theta^{\mathrm{\small open}}$, we use the prediction from i=1 at inference time. Our objective reads:

%\vspace{-0.1in}
\small 
\begin{align}
    \mathcal{L}_\theta =  w_1 \|(\epsilon_\theta^{\mathrm{\small loc}}(\oo, l, c,\tr^i,i) - \epsilon^{\mathrm{\small loc}}\| + w_2 \|(\epsilon_\theta^{\mathrm{\small rot}}(\oo, l, c,\tr^i,i) - \epsilon^{\mathrm{\small rot}}  \| + \mathrm{BCE}(f_\theta^{\mathrm{\small open}}(    \oo, l, c,\tr^i,i),\mathbf{a}_{1:T}^{\mathrm{\small open}}) ,
    \nonumber
\end{align}
%\vspace{-0.1in}

\normalsize

where $w_1,w_2$ are hyperparameters estimated using cross-validation.  
To draw a sample from the learned distribution $p_\theta(\tr|\oo,\lang, \hist)$, we start by drawing a sample $\tr_\maxid\sim\mathcal{N}(\mathbf{0},\mathbf{1})$. 
Then, we progressively denoise the sample by iterated application of $\epsilon_{\theta}$ $\maxid$ times according to a specified sampling schedule~\cite{DDPM,song2020denoising}, which terminates with $\tr_0$ sampled from $p_\theta(\tr)$: 
%\begin{align}
$\tr^{i-1} = \frac{1}{\sqrt{\alpha^{i}}} \left( \tr^i - \frac{\beta^i}{\sqrt{1-\bar{\alpha}_i}} \epsilon_\theta(\oo,l,c,\tr^i,i) \right)
+ \frac{1 - \bar{\alpha}^{i+1}}{1 - \bar{\alpha}^{i}}\beta^{i} \mathbf{z},$ 
%\nonumber
%\end{align}
where $\mathbf{z}\sim \mathcal{N} (\bzero,\bone) $ is a random variable of appropriate dimension.  Empirically, we found that using separate noise schedulers for $\ac^{\mathrm{\small loc}}$ and $\ac^{\mathrm{\small rot}}$, specifically, scaled-linear and square cosine scheduler, respectively, achieves better performance. 
%We also include a detailed model diagram and a table of hyper-parameters  in Section~\ref{sec:details} and ~\ref{sec:hyper_parameter} of the Appendix.

%In order to draw a sample from the learned distribution $p_\theta(\tr|\oo,\lang, \hist)$, we start by drawing a sample $\tr_\maxid\sim\mathcal{N}(\mathbf{0},\mathbf{1})$. 
%Then, we progressively denoise the sample by iterated application of %$\epsilon_{\theta}$ $\maxid$ times according to a specified sampling schedule~\cite{DDPM,song2020denoising}, which terminates with $\tr_0$ sampled from %$p_\theta(\tr)$: 
%\begin{equation} \label{eq:diffupdate}
%x_{\id-1} = \frac{1}{\sqrt{\alpha_{\id}}} \left( x_\id - \frac{\beta_\id}{\sqrt{1-%\bar{\alpha}_\id}} \epsilon_\theta (x_\id,\id,\cond) \right) +\frac{1 - %\bar{\alpha}_{\id+1}}{1 - \bar{\alpha}_{\id}}\beta_{\id} \mathbf{z},
%\end{equation}
%where $\mathbf{z} \sim \mathcal{N} (\bzero,\bone)$.

\noindent \textbf{Implementation details} 
At training, we segment demonstration trajectories at detected end-effector \textit{keyposes}, such as a change in the open/close end-effector state or local extrema of velocity/acceleration, following  previous works \cite{james2022q, shridhar2023perceiver, gervet2023act3d, liu2022instruction}. We then resample each trajectory segment to have the same length $T$. %\modellong{} is trained to predict the resampled trajectories. 
During inference, \model{} can either predict and execute the full trajectory of actions up to the next keypose (including the keypose), or just predict the next keypose and use a sampling-based motion planner to reach it, similar to previous works \cite{shridhar2023perceiver,guhur2023instruction,gervet2023act3d}.
%In the rest of this section we use the term ``trajectory" to refer to \model{}'s output. 

Due to space limits, please check Section~\ref{sec:details} for detailed model diagram, Section~\ref{sec:hyper_parameter} for our choice of hyper-parameters, Section~\ref{subsec:diffusion_prelim} for detailed formulation of denoising diffusion probabilistic models and Section~\ref{sec:squaredcos} for discussion of noise schedulers in the Appendix. 
\begin{comment}


We augment RGB-D observations with random rescaling and cropping.  Nearest neighbor interpolation is used for rescaling RGB-D observations. 
To reduce the memory footprint in our 3D Relative Transformer, we use Farthest Point Sampling to sample a subset of the points in the input 3D feature cloud.  We use FiLM~\cite{perez2018film} to inject conditional input, including the diffusion step and proprioception, to every attention layer in the model. We include a detailed architecture diagram of our model and a table of hyper-parameters used in our experiments in the Appendix (Section~\ref{sec:details} and Section~\ref{sec:hyper_parameter}). 


\noindent \textbf{Keyposes} \model{} inherits the temporal abstraction of demonstrations into end-effector \textit{keyposes} from previous works \cite{james2022q, shridhar2023perceiver, gervet2023act3d, liu2022instruction}. Keyposes are important intermediate end-effector poses that summarize a demonstration and can be extracted using simple heuristics, such as a change in the open/close end-effector state or local extrema of velocity/acceleration. 
%We describe the heuristics we use for each dataset in the Appendix (Section~\ref{sec:heuristics_calvin}). 
During inference, \model{} can either predict and execute the full trajectory of actions up to the next keypose (including the keypose), or just predict the next keypose and use a sampling-based motion planner to reach it, similar to previous works \cite{shridhar2023perceiver,guhur2023instruction,gervet2023act3d}. In the rest of this section we use the term ``trajectory" to refer to \model{}'s output. Keypose prediction is a special case where the trajectory contains  only one future pose. \fixme{probably separate this section to different experiment subsections.} 

\end{comment}

==> 5_exps_new.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experiments}
\label{sec:experiment}
\vspace{-0.1in}
We test \model{} in  multi-task manipulation  on RLBench \cite{james2020rlbench} and CALVIN \cite{mees2022calvin}, two established learning from demonstrations benchmarks, and in the real world.  %We compare against state-of-the-art methods on single-view and multi-view setups, as well as against ablative versions of our model that do not consider 3D scene representations or relative attention. %We also test \model{}'s ability to learn multi-task policies from real-world demonstrations. 


% \input{src/fig_task.tex}

\vspace{-0.1in}
\subsection{Evaluation on RLBench}
\vspace{-0.1in}
%\noindent \textbf{Setup}
RLBench is built atop the CoppelaSim~\cite{rohmer2013v} simulator, where a Franka Panda Robot is used to manipulate the scene. 
On RLBench,  our model and   all  baselines are trained to predict the next end-effector keypose as opposed to keypose trajectory;  all methods employ a low-level motion planner BiRRT~\cite{kuffner2000rrt}, native to RLBench, to reach the predicted robot keypose. %During motion planning, Our model does not perform collision checking for our experiments. 
We train and evaluate \model{} on two setups based on the number of available cameras:    \textbf{1.} \textit{Multi-view setup}, introduced in \cite{shridhar2023perceiver}, that uses a suite of 18 manipulation tasks, each with 2-60 variations, which concern scene variability across object poses, appearance and semantics. 
    %The tasks are specified by language descriptions. 
    There are  four RGB-D cameras available, front, wrist, left shoulder and right shoulder. The wrist camera moves during manipulation.  
   % There are 100 training demonstrations  per task, evenly split across task variations, and 25 (unseen) test episodes for each task.  During evaluation, models are allowed to predict a maximum temporal horizon of 25 keyposes, unless they receive earlier task-completion indicators from the simulation environment. Due to the randomness of the sampling-based motion planner, we test our model across 5 random seeds.
   \textbf{2.} \textit{Single-view setup}, introduced in \cite{ze2023gnfactor}, that  
     uses a suite of 10 manipulation tasks. Only the front RGB-D camera view is available. 
     %There are 20 training demonstrations per task, evenly split across variations.  We still use same 25 test episodes and horizon of 25 keyposes, with the exception that we test the final checkpoint using 3, rather than 5, random seeds on the test set.
    We evaluate policies by task completion success rate, which is the proportion of execution trajectories that achieve the goal conditions specified in the language instructions \cite{gervet2023act3d,shridhar2023perceiver}.
%\end{enumerate}

%\todo{tsung-wei says 3d policies use camera extrinsics-INTRO}
\noindent \textbf{Baselines} 
All compared methods on RLBench are 3D policies that use depth and camera parameters during featurization of the  RGB-D input. 
We compare against the following: C2F-ARM-BC~\cite{james2022coarse} and PerAct~\cite{shridhar2023perceiver} that voxelize the 3D workspace, Hiveformer~\cite{guhur2023instruction} that featurizes XYZ coordinates aligned with the 2D RGB frames,  PolarNet~\cite{Chen2023PolarNet3P} that featurizes a scene 3D point cloud, GNFactor~\cite{ze2023gnfactor} that uses a single RGB-D view and is trained to complete the 3D feature volume, RVT~\cite{goyal2023rvt} and Act3D ~\cite{gervet2023act3d}, that are the previous SOTA methods on RLBench. 
We report results for RVT, PolarNet and GNFactor based on their respective papers. Results for CF2-ARM-BC and PerAct are presented as reported in \cite{goyal2023rvt}. Results for Hiveformer are copied from \cite{Chen2023PolarNet3P}. We retrained Act3D on the multi-view setup using the publicly available code, because we found some differences on the train and test splits used in the original paper. We also trained  Act3D on the single-view setup to use as additional baseline for the single-view setup, alongside GNFactor. \model{} and all  baselines are trained on the same set of keyposes extracted from expert demonstrations~\cite{james2022q}.  %For more details on the baseline description, please check Section~\ref{sec:baselines} of the Appendix 

\begin{comment}
We consider the following baselines: 
    \textbf{1.} C2F-ARM-BC~\cite{james2022coarse}, a 3D policy that iteratively voxelizes RGB-D images and predicts actions in a coarse-to-fine manner. Q-values are estimated within each voxel and the translation action is determined by the centroid of the voxel with the maximal Q-values. 
    \textbf{2.} PerAct~\cite{shridhar2023perceiver},  a 3D policy that voxelizes the workspace and detects the next voxel action through global self-attention.  
    \textbf{3.} Hiveformer~\cite{guhur2023instruction}, a 3D policy that enables attention between features of different history time steps. 
    \textbf{4.} PolarNet~\cite{Chen2023PolarNet3P}, a 3D policy that computes dense point representations for the robot workspace using a PointNext backbone \cite{Qian2022PointNeXtRP}. 
    \textbf{5.} RVT~\cite{goyal2023rvt}, a 3D policy that deploys a multi-view transformer to predict actions and fuses those across views by back-projecting to 3D. 
    \textbf{6.} Act3D ~\cite{gervet2023act3d}, a 3D policy that featurizes the robot's 3D workspace using coarse-to-fine sampling and featurization. We observed that Act3D~\cite{gervet2023act3d} does not follow the same setup as PerAct on RLBench. Specifically, Act3D uses different 1) 3D object models, 2) success conditions, 3) training/test episodes and 4) maximum numbers of keyposes during evaluation.  For fair comparison, we retrain and test Act3D on the same setup.
%\textbf{5.} InstructRL~\cite{liu2022instruction}, a 2D policy that directly predicts 6 DoF poses from image and language conditioning with a pre-trained vision-and-language backbone.
    \textbf{7.} GNFactor~\cite{ze2023gnfactor}, a 3D policy that co-optimizes a neural field for reconstructing the 3D voxels of the input scene and a PerAct module for predicting actions based on voxel representations.
\end{comment}



%We observed that Act3D~\cite{gervet2023act3d} does not follow the same setup as PerAct on RLBench. Specifically, Act3D uses different 1) 3D object models, 2) success conditions, 3) training/test episodes and 4) maximum numbers of keyposes during evaluation.  For fair comparison, we retrain and test Act3D on the same setup.



%\noindent \textbf{Evaluation metrics} 



\input{src/tab_peract}
\input{src/tab_gnfactor}
%\noindent \textbf{Results on the  Multi-View setup} 
We show quantitative results for the multi-view setup in Table~\ref{tab:peract} and for single-view setup in Table~\ref{tab:gnfactor}. On multi-view, \model{} %outperforms all baselines on most tasks by a large margin. It
achieves an average $81.3\%$ success rate among all 18 tasks, an absolute improvement of $+18.1\%$ over Act3D, the previous state-of-the-art.  In particular, \model{} achieves big leaps on long-horizon high-precision tasks with multiple modes, such as {\it stack blocks}, {\it stack cups} and {\it place cups}, which most baselines fail to complete. 
All  baselines use classification or regression losses, our model is the only one to use diffusion for action prediction.   

%We obtain substantial improvements of $+39.5\%$, $+18.4\%$, $+41.6\%$ and $+20.8\%$ on {\it stack blocks}, {\it put in cupboard}, {\it insert peg} and {\it stack cups} respectively.  %Notably, the original success condition for the {\it close jar} task, as defined by PerAct's RLBench library, is incorrect, leading to failure in all expert demonstrations. We report our results using the corrected success condition proposed in this pull request\footnote{https://github.com/MohitShridhar/RLBench/pull/1}.
%\noindent \textbf{Results on the GNFactor setup} 
%We show quantitative results in Table~\ref{tab:gnfactor}. %We train Act3D on this setup using its publicly available code. 
%\footnote{https://github.com/zhouxian/act3d-chained-diffuser}. 
On single-view, \model{} outperforms  GNFactor by $+46.7\%$ and Act3D by $+13.1\%$. Surprisingly, Act3D also outperforms GNFactor by a big margin. This  suggests that the choice of 3D scene representation is more crucial than 3D feature completion. 
Since Act3D has a similar 3D scene tokenization as \model{}, this shows the importance of diffusion over alternatives to handle multimodality in prediction, specifically over sampling based 3D action maps and rotation regression.  

%We re-trained Act3D for this single view setup.  Notably, \model{} and Act3D utilize similar 3D scene representations, sparse 3D feature tokens, while GNFactor featurizes a scene with 3D voxels and learns to reconstruct them across views. Even with a single camera view, both Act3D and \model{} outperform GNFactor significantly. This  suggests that the choice of 3D scene representation is a more crucial factor than the completion of 3D scenes in developing efficient 3D manipulation policies.


\noindent \textbf{Ablations} 
We  consider the following ablative versions of our model:  
%\begin{enumerate}
%\item
\textbf{1.} \textrm{2D Diffuser Actor}, our implementation of 2D Diffusion Policy of \cite{chi2023diffusion}.  We remove the 3D scene encoding from \model{} and instead  use per-image 2D representations by average-pooling features within each view.  We  add learnable embeddings to distinguish between different views and fuse them with action estimates, as done in \cite{chi2023diffusion}.  %We use standard attention layers for joint encoding the action estimate and 2D image features.
\textbf{2.} \model{} w/o RelAttn., an ablative version that uses absolute (non-relative) attentions. %This version of our model is not translation equivariant.
%\end{enumerate}
\input{src/tab_ablation}


We show ablative results  %design choices of \model{}, specifically 
%the use of 3D scene representations and the use of relative attentions  in the PerAct experimental setup 
in Table \ref{tab:ablation}.  %\todo{wrap table}
%We use the PerAct experimental setup. 
%We draw the following conclusions: 
%\textbf{1.} 
\modellong{} largely outperforms its 2D counterpart, 2D Diffuser Actor. This shows the importance of 3D scene representations in performance.  
%\textbf{2.} 
\modellong{} with absolute 3D attentions (3D Diffuser Actor w/o RelAttn.) is  worse than \modellong{} with relative 3D attentions. This shows that translation equivariance through relative attentions is  important for generalization. Despite that, this ablative version already outperforms all prior arts in Table~\ref{tab:peract}, proving the effectiveness of marrying 3D representations and diffusion policies.



\subsection{Evaluation on CALVIN} 
\vspace{-0.1in}
%\noindent \textbf{Setup}
The CALVIN benchmark  is built on top of the PyBullet~\cite{coumans2016pybullet} simulator and involves a Franka Panda Robot arm that manipulates the scene. CALVIN consists of 34 tasks and 4 different environments (A, B, C and D). All environments are equipped with a desk, a sliding door, a drawer, a button that turns on/off an LED, a switch that controls a lightbulb and three different colored blocks (red, blue and pink).  These environments differ from each other in the texture of the desk and positions of the objects.  CALVIN provides 24 hours of tele-operated unstructured play data, 35\% of which are annotated with language descriptions.  
Each instruction chain includes five language instructions that need to be executed sequentially. We evaluate on the so called \textit{zero-shot generalization  setup}, where models are trained in environments A, B and C and tested in D. We report the success rate and the average number of completed sequential tasks, following previous works \cite{mees2022hulc,wu2023unleashing}. No motion planner is available in CALVIN so all models need to predict robot pose trajectories.   

 

\noindent \textbf{Baselines}   
%We compare against multiple previous works. 
All methods tested so far in CALVIN are 2D policies, that do not use depth or camera extrinsics. 
We compare against the hierarchical 2D policies of MCIL~\cite{lynch2020language}, HULC~\cite{mees2022hulc} and  SuSIE~\cite{black2023zero} which predict latent features or images of  subgoals given a language instruction, which they feed into lower-level subgoal-conditioned policies.
They can train the low-level policy on all data available in CALVIN as opposed to the language annotated subset only. We compare against large scale 2D transformer policies of  RT-1~\cite{brohan2022rt},  RoboFlamingo~\cite{li2023vision} and GR-1~\cite{wu2023unleashing} which pretrain on large amounts of interaction or observational (video alone) data. We report results for HULC, RoboFlamingo, SuSIE and GR-1 from the respective papers. Results from MCIL are borrowed from \cite{mees2022hulc}. Results from RT-1 are copied from \cite{wu2023unleashing}. 

We also compare against 3D Diffusion Policy~\cite{Ze2024DP3} and ChainedDiffuser \cite{xian2023chaineddiffuser}, which we train both on the language annotated training set. 
%that uses holistic 3D scene pointcloud embeddings and
%. Last, we also compare against a 3D policy of ChainedDiffuser that uses Act3D to predict keyposes and diffusion models to link the current and predicted keypose. 
We evaluate 3D Diffusion Policy, ChainedDiffuser and \model{} with the final checkpoints across 3 seeds.
We report both the mean and standard deviation of evaluation results.  We devise an algorithm to extract keyposes on CALVIN, since prior works do not use keyposes.  We define keyposes as those at frames with significant motion change.  Both ChainedDiffuser and \model{} segment the demonstations based on the keyposes.
%are trained to predict keyposes and corresponding trajectories to reach each keypose. 
Notably, though keyposes extracted in RLBench have clear structure since they correspond to programmatically labeled  3D waypoints~\cite{james2020rlbench,james2022q},    keyposes extracted in CALVIN are instead noisy and random, as the benchmark consists of human play trajectories.
%We train \modellong{}  on the subset of play data annotated with language descriptions on the environments A, B and C and  evaluate it on 1000 unique instruction chains on environment D, following~\cite{li2023vision,wu2023unleashing}.  
%Please, check Section~\ref{sec:baselines} and ~\ref{sec:dp3_calvin} of the Appendix for more details.




For evaluation, prior works~\cite{mees2022hulc,black2023zero,li2023vision} predict a maximum temporal horizon of 360 actions to complete each  task, while, on average,  ground-truth trajectories are only 60 actions long.  Our model predicts trajectories and replans after each trajectory has been executed, instead of after each individual actions. On average, it takes 10 trajectory inference steps to complete a task. We thus allow our model to predict a maximum temporal horizon of 60 trajectories for each task. 


%For reference, we also allow our model to predict 360 times (last row in Table \ref{}). % and show the influence of this hyperparameter in the Appendix (Section~\ref{sec:curve_calvin}).


\input{src/tab_calvin}

%\noindent \textbf{Evaluation metrics} 



%\noindent \textbf{Results} 
We show quantitative results in Table~\ref{tab:calvin}. \model{} outperforms  %competitive results compared to 
the state-of-the-art. % In comparison to GR-1, our model achieves absolute performance gains of \rebut{$+6.8\%$, $+9.1\%$, $+6.6\%$, $3.6\%$ and $+1.1\%$} for completing the 5 tasks in the instruction chain.  On average, \model{} complete \rebut{$3.35$} tasks in a row, setting a new state of the art. 
%In this benchmark, , as a result,
ChainedDiffuser does not work well on this benchmark. The reason is that its deterministic keypose prediction module fails to predict end-effector keyposes accurately due to multimodality present in human demonstrations of CALVIN in comparison to programmatically collected demonstrations of RLBench. 
%, completing only $0.84$ tasks in a row.}. 
%Note that GR-1's contribution is large-scale pre-training on videos, which is a scheme orthogonal to our contribution. 
Allowing \modellong{} to have a longer horizon before terminating increases the performance significantly, which suggests that the model learns to retry under failure. 
%For this performance, we found stronger conditioning on the language instructions to be important, as we explain in our appendix (Figure~\ref{fig:detailed_diagram}b).


%\todo{wrap table}
\input{src/tab_real}
\subsection{Evaluation in the real world}
We validate  \model{} in learning manipulation tasks from real-world demonstrations across 12 tasks.  We use a Franka Emika robot equipped with a Azure Kinect RGB-D sensor at a front view.  Images are originally captured at $1280 \times 720$ resolution and downsampled to a resolution of $256 \times 256$.  %Camera extrinsics are calibrated w.r.t the robot base. 
During inference, we utilize the BiRRT~\cite{kuffner2000rrt} planner provided by the MoveIt! ROS package \cite{coleman2014reducing} to reach the predicted poses. %We use 12 tasks 
\begin{comment}
1) {\it close a box}, 2) {\it put ducks in bowls}, 3) {\it insert a peg vertically into the hole}, 4) {\it insert a peg horizontally into the torus}, 5) {\it put a computer mouse on the pad}, %6) {\it rotate and open the bottle cap}, 
6) {\it open the pen}, 7) {\it press the stapler}, 8) {\it put grapes in the bowl}, %10) {\it align the screwdriver parallel to tools}, 
9) {\it sort the rectangle}, 10) {\it stack blocks with the same shape}, 11) {\it stack cups} and 12) {\it put block in a triangle on the plate}. Details on the task definitions and success criteria are included in the Appendix (Section~\ref{sec:real_world_tasks}).
\end{comment}
We collect 15 demonstrations per task, most of which naturally contain noise and multiple modes of human behavior. For example, we pick one of two ducks to put in the bowl, we insert the peg into one of two holes and we put one of three grapes in the bowl. %, as shown in Figure \ref{fig:real}.
%\model{} conditions on language descriptions and is trained to predict the next end-effector keypose.
 We evaluate 10 episodes for each task and report the success rate.  
We show quantitative results in Table~\ref{tab:real} and video results on our project webpage. \modellong{}  effectively learns real-world manipulation from a handful of demonstrations. 



% \input{src/tab_runtime}
\noindent \textbf{Runtime} We compare the control frequency of our model against ChainedDiffuser \cite{xian2023chaineddiffuser} and 3D Diffusion Policy \cite{Ze2024DP3} on CALVIN, using an NVIDIA 2080 Ti graphic card.  The inference speed of \model{}, ChainedDiffuser and 3D Diffusion Policy is 600ms, 1170ms (50 for keypose detection and 1120 for trajectory optimization) and 581ms for executing 6, 6 and 4 end-effector poses. The respective control frequency is 10 Hz, 5.1 Hz and 5.2 Hz. %Notably, out of the 1170 ms for ChainedDiffuser, only 50 ms are for keypose detection Act3D \cite{gervet2023act3d}
%\paragraph{More analyses} 



\paragraph{Limitations}
\label{subsec:limitation}
Despite its SOTA performance with large margins over existing methods, %our model has limitations. 
our framework currently has the following limitations: 
{\bf 1.} It requires camera calibration and depth information, same as all 3D policies. 
{\bf 2.} All tasks in RLBench and CALVIN are quasi-static. Extending our method to dynamic tasks and velocity control is a direct avenue of future work. 
{\bf 3.} It is on average slower than non-diffusion policies. This can be improved by recent techniques on reducing the inference steps of diffusion models.


Please, refer to our Appendix for more experiments and details: Section ~\ref{sec:noisy_depth} for robustness of \modellong{} to depth noise, Section~\ref{sec:failure} for discussion of failure cases, Section~\ref{sec:rlbench_tasks} and ~\ref{sec:real_world_tasks} for descriptions of tasks in RLBench and the real world, Section \ref{sec:baselines} for descriptions of baselines, Section~\ref{sec:dp3_calvin} for implementation details of re-training 3D Diffusion Policy on CALVIN, Section~\ref{sec:heuristics_calvin} for keypose discovery on CALVIN. Video results can be found in our supplementary file.

==> 6_conclusion.tex <==
\section{Conclusion}
\label{sec:summary}
We present \modellong{}, a  manipulation policy that combines 3D scene representations and action diffusion. Our method sets a new state-of-the-art on RLBench and CALVIN by a large margin  over existing 2D and 3D policies, and learns robot control in the real world from a handful of demonstrations. \model{} builds upon recent progress on 3D tokenized scene representations for robotics and on generative models and shows how their combination is a powerful learning from demonstration method. Our future work includes learning \model{} policies from suboptimal demonstrations and scaling up training data in simulation and in the real world.    
%that employ large-scale video pre-training. 
%We introduce important architectural innovations, such as 3D token representations of the robot's pose estimate and 3D relative position denoising transformers that endow \modellong{} with translation equivariance, and empirically verify their contribution to performance. 
%We further test our model in the real world and show it can learn  manipulation tasks from a handful of demonstrations. 
%renders the current estimate of the robot's end-effector in its estimated 3D position and orientation, and featurizes it with relative 3D attention layers to predict the residual error (noise). 
 
 %Our future work will attempt to train  \modellong{} policies  in domain-randomized simulation environments at a large scale, to help them transfer  from simulation to the real world. 
%The denoising process obtaines iterative error feedback on the predictions of the end effector. 

%, to presenve translation invariance. Our model 


==> 7_misc.tex <==
% \subsubsection*{Author Contributions}
% If you'd like to, you may include  a section for author contributions as is done
% in many journals. This is optional and at the discretion of the authors.

\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.
\fixed{Add Moritz Reuss, very helpful for CALVIN experiments (relative action and weight decay)}

==> rss_tex/9_rebuttal.tex <==
\clearpage
\newcommand{\sofn}[1]{{\color{cyan}SoFn}}
\newcommand{\rttc}[1]{{\color{purple}rTTc}}
\newcommand{\gyzr}[1]{{\color{blue}GyZr}}

\noindent We thank the reviewers for their feedback on our paper. All reviewers appreciate our ``thorough experimental evaluations" (\sofn{}), with ``large amounts of ablations on a variety of simulation benchmarks" (\rttc{}) and ``a lot of hardware experiments" (\rttc{}), that ``show strong performance (SOTA)" (\gyzr{}) ``on established multi-task benchmarks" (\sofn{}), ``offering valuable insights for future research and development" (\sofn{}). We address the reviewers concerns below. We updated the paper to incorporate the reviewers' feedback. The updated passages are marked with \color{orange}orange \color{black}text.

\input{src/fig_method_comparison}
\noindent \textbf{How does 3D Diffuser Actor combine the different feature maps from different images? (\sofn{}) What is the representation of the 3D data when fed to the policy? (\rttc{})} 
To clarify the input form and representation, we updated the paragraph ``Scene and language encoder" in the method section as follows:

We use a scene and language encoder similar to \cite{gervet2023act3d,xian2023chaineddiffuser}. We describe it here to make the paper self-contained. 
The input to our scene encoder is a set of posed RGB-D images, captured from cameras with known extrinsic and intrinsic parameters. Each RGB image is a tensor $I_{c_i} \in \mathbb{R}^{H\times W\times 3}$, where $H, W$ the height and width respectively in pixels, $c_i$ the camera indicator. Each depth image is a tensor $D_{c_i} \in \mathbb{R}^{H\times W}$. We use the camera parameters, the depth map $D_{c_i}$ and the pinhole camera equation to obtain a 3D location map $P_{c_i} \in \mathbb{R}^{H\times W\times 3}$ for every pixel: essentially we map each pixel location and depth value $(x,y,d)$ to a 3D location $(X,Y,Z)$.

We feed each camera observation $I_{c_i}$ separately to a pre-trained 2D feature extractor to get a subsampled feature map $f_{c_i} \in \mathbb{R}^{H'\times W'\times F}$, with $F$ the feature dimension. For each 3D location map $P_{c_i}$ we run a local average pooling to get a subsampled location map of shape $P'_{c_i} \in \mathbb{R}^{H'\times W'\times 3}$. We stack all feature maps into a tensor in $\mathbb{R}^{N_c\times H'\times W'\times F}$, where $N_c$ is the number of cameras. We then reshape to obtain a feature cloud of shape $\mathbb{R}^{N_cH'W'\times F}$. This is invariant to the order of cameras and no camera identity information is needed. We follow the same the procedure to obtain the associated 3D locations in $\mathbb{R}^{N_cH'W'\times 3}$.
As $(N_c H' W')$ can be a large number and, as a result, computationally expensive to handle in the attention layers, we run Farthest Point Sampling to select a subset of $N_p$ points in the 3D feature cloud. This leads to a scene representation as a feature cloud $Z_o \in \mathbb{R}^{N_p \times F}$, associated with 3D locations in $\mathbb{R}^{N_p \times 3}$.


The language encoder maps language task descriptions or instructions into language feature tokens $Z_l \in \mathbb{R}^{N_L \times F}$. We use the pre-trained CLIP ResNet50 2D image encoder ~\cite{radford2021learning} to encode each RGB image into a 2D feature map and the pre-trained CLIP language encoder to featurize the  language task instruction.

\noindent \textbf{More implementation details? (\rttc{})} In addition to more details on the scene and language representation (see previous question), we extended the paragraph ``3D Relative Position Denoising Transformer" as follows:

3D Diffuser Actor iteratively denoises an estimate of the end-effector's future trajectory. Every trajectory step token is a 10-dimensional action, as defined earlier. We project each such action into a high-dimensional representation through an MLP to obtain a trajectory representation $Z_T \in \mathbb{R}^{N_T \times F}$, with $N_T$ the number of trajectory tokens. Each action token comes with the positional embeddings of its corresponding $\ac^{\mathrm{\small pos}}$. This enables relative cross-attention with the scene and other physical entities. 
We incorporate proprioceptive information as a short, fixed-length history of predicted end-effector keyposes. These are represented with learnable feature vectors $Z_c \in \mathbb{R}^{N_h \times F}$, where $N_h$ the history length, and their 3D positions are used to compute positional embeddings.

% We contextualize all tokens, namely visual $o$, language $l$, proprioception $c$ and action tokens (current estimate) $\ac_t^{pos}, \ac_t^{rot}$
We contextualize all tokens, namely visual $Z_o$, language $Z_l$, proprioception $Z_c$ and action tokens (current estimate) $Z_T$ using 3D relative position attention layers. Specifically, the scene tokens $Z_o$ first attend to the language tokens $Z_l$. Then, the trajectory tokens $Z_T$ attend to the updated scene tokens $Z'_o$. Lastly, we concatenate the updated trajectory $Z'_T$ and scene tokens $Z'_o$ along the sequence dimension and feed to self-attention layers. The proprioception tokens and the denoising step are used as conditional inputs to every attention layer in the model using the FiLM technique \cite{perez2018film}.

\noindent \textbf{Is the history end-effector poses of variable length? Does the length affect in any manner? What are the history end-effector poses for the first prediction? (\sofn{})}
The history of end-effector poses has a fixed length of 3 in all our experiments. We updated our paper to clarify this. For the first timesteps where we don't yet have a long enough history we simply pad with the initial end-effector pose. \todo{result}

\noindent \textbf{Two actions, that have similar $a_{pos}$ but different orientations will have similar positional embeddings? (\sofn{})}
Yes, this is correct. Note though that the action features already contain the rotation information. As we describe in our paper: ``Every trajectory step token is an 10-dimensional action, as defined earlier. We project each such action into a high-dimensional representation through an MLP".

\noindent \textbf{The figures lack implementation details to help understand the differences from PerAct and Act3d. (\rttc{})}
We refer to Figure~\ref{fig:compare} that illustrates the difference between \model{} and other methods.

\noindent \textbf{Relation of 3D Diffuser Actor to Act3D. (\rttc{})}
Act3D is a method that learns from demonstrations to predict 3D keyposes of the robot's end-effector, conditioned on multiview RGB-D images and a language instruction. Its goal is to predict a 3D action map \todo{write the dimensions!}so that it preserves equivariance, which helps generalization in action prediction. Main contribution: A high resolution 3D action map typically requires a high resolution 3D voxel grid to featurize. This is a problem since it is prohibitively expensive to run all-to-all attentions across all 3D voxels. Act3D foregoes 3D voxelization altogether and instead uses a coarse-to-fine 3D point sampling and featurization, to build 3D action maps of varying 3D spatial resolution (we say this in our related work: ``Act3D \cite{gervet2023act3d} foregoes 3D scene voxelization altogether; it instead computes a 3D action map of variable spatial resolution by sampling 3D points in the empty workspace and featurizing them using cross-attentions to the 3D physical points."). Details: Act3D instantiates a scene 3D feature cloud by featurizing multiview RGB images and lifting the patch features to 3D using sensed depth. It also encodes the language instruction using CLIP's language encoder. It then samples 3D points (they call them ghost points) on a 3D grid and featurize them by cross-attending to the scene 3D feature cloud. The scene 3D feature cloud is never updated. A learnable query also cross-attends to the scene feature cloud and it is used to score all 3D ghost points and predict a 3D action map in this way. This process is repeated 3 times, each time with a refined 3D ghost point sampling and more fine-grained visual features to improve map resolution. At the end, the query features are also used to regress to a 3D rotation of the end-effector.  See Figure~\ref{fig:act3d_detailed_diagram} in the Appendix for the detailed diagram of Act3D.

3D Diffuser Actor is a method that learns to predict 3D keyposes of the robot's end-effector conditioned on multiview RGB-D images and a language instruction using learning from demonstrations (this is identical to Act3D). It foregoes predicting 3D action maps altogether. Its bet is that the iterative denoising process will be able to handle multimodality in 3D end-effector location better than 3D action maps, while in addition handling multimodality in 3D rotation (in Act3d rotation is simply regressed). The hope is that these two will lead to better generalization in 3D keypose prediction. Main contribution: 3D Diffuser Actor casts 3D keypose prediction as a denoising process conditioned on multiview images and language instructions. It proposes a denoising network that takes as input multiview images, a language instruction, a current estimate of the end effector’s 3D rotation and 3D translation and the index of the denoising iteration of diffusion, and outputs the noise in the 3D translation and rotation of the end effector. It featurizes the RGB multiview images using a 2D pretrained backbone (CLIP) and lifts the 2D feature maps into a 3D featured cloud. It then embeds the language instruction using a CLIP language encoder (similar to Act3D and CLIPort among others), it uses FiLM layers to input the denoising iteration and instantiates a 3D token for the current end-effector estimate. It uses relative 3D position attentions to fuse all this information (we cite Act3D as an inspiration for that). 3D Diffuser's Actor 3D relative transformer is very different from Act3D's: 3D Diffuser Actor does not use 3D ghost point grids or coarse-to-fine featurizations. The noisy keypose token, visual tokens and proprioception tokens are fed to a 3D relative self-attention layer that also updates the scene feature tokens. We refer to our Figure~\ref{fig:detailed_diagram} in the Appendix for an illustration of our denoising 3D transformer model.

The models of Act3D and 3D Diffuser Actor are thus different in that:
\begin{itemize}
    \item One is a diffusion model the other is a deterministic model.

    \item They have different inputs and outputs as noted above. One maps x to y directly through coarse to fine 3D point sampling for 3D location and regression for 3D rotation, the other is a denoising diffusion model that takes x and the current y estimate (3D location and 3D rotation) and iteration index and predicts the noise in the current estimate.

    \item There is no coarse-to-fine sampling or any form of point sampling in 3D Diffuser Actor.

    \item 3D Diffuser Actor does not build a 3D map (a map of 3D locations where each one is scored whether it contains the next end-effector 3D keypose or not).

    \item The 3D relative transformers differ as noted above: 1) the token sets are very different as explained above, 2) one is a cross-attention and the other a self-attention.
\end{itemize}


\noindent \textbf{Relation of 3D Diffuser Actor to ChainedDiffuser. (\rttc{})}
ChainedDiffuser is a method that takes as input 3D keyposes predicted by Act3D and predicts end-effector trajectories to link the current keypose to the predicted one. Main contribution: ChainedDiffuser proposes to get rid of sampling-based motion planners (like RRT) because they fail in tasks that cannot be easily decomposed into straight-line trajectory segments, such as opening doors or wiping the table, and instead uses trajectory diffusion that conditions on the current and predicted 3D end-effector keyposes to predict a 3D end-effector trajectory that links them.

Details: ChainedDiffuser uses an architecture similar to Act3D to create a 3D feature cloud and takes as input the current trajectory estimate to predict scaled noise for translation trajectory and the final denoised rotation trajectory. It shows that in tasks that require continuous motion, Act3D keyposes in combination with this trajectory denoising from keypose to keypose, much outperforms Act3D+motion planners. ChainedDiffuser’s contribution is a learnt trajectory predictor that works alongside an off-the-shelf 3D keypose prediction method. ChainedDiffuser is complementary to our work: We can use keyposes predicted by 3D Diffuser Actor and link them with ChainedDiffuser’s trajectories instead of motion planners and achieve similar boosts in these tasks. Because the tasks in the PerAct benchmark that we consider do not require such continuous trajectories, motion planners work well, so we did not use a trajectory prediction model.%; ChainedDiffuser performs as well as Act3D there (no additional performance boost).

The diffusion models of ChainedDiffuser and 3D Diffuser Actor are thus different in that: 1. ChainedDiffuser takes as input the to-reach 3D keypose while 3D Diffuser Actor tries to predict it. In that sense, 3D Diffuser Actor has a much much harder task to solve. \fixme{2. 3D Diffuser Actor denoises 3D keyposes and trajectories and ChainedDiffuser denoises 3D trajectories.} 3. The experiments in ChainedDiffuser concern single manipulation tasks while 3D Diffuser Actor shows multi-task results across the whole PerAct suite.

The models of ChainedDiffuser and 3D Diffuser Actor are similar in that:

Both build 3D feature clouds and use diffusion to predict their desired output, being the next 3D keypose for 3D Diffuser Actor and being a current to predicted 3D keypose trajectory for ChainedDiffuser.
ChainedDiffuser can take as input the keyposes predicted by 3D Diffuser Actor and we explained above why we did not consider this.

\noindent \textbf{In the conclusion, the authors mention that the 3D relative position denoising transformers is a technical contribution of this work. Is that right. Was this concept not introduced in Act3D and its importance also shown in that paper? (\sofn{})}
\todo{}

\noindent \textbf{Show standard deviations? It looks like there are often tasks are often better with Act3D. (\rttc{})} In our original submission we included the standard deviation for all methods that report it in their papers. We additionally updated Table~\ref{tab:gnfactor} and Table~\ref{tab:calvin} with standard deviations of success rates evaluated across multiple random seeds. Even if Act3D achieves competitive performance on some tasks, 3D Diffuser Actor vastly outperforms it on most of the tasks. In RLBench, on average across 5 random seeds our method outperforms Act3D by 18.1\%.

\noindent \textbf{Why only 2D policies as comparisons on CALVIN benchmark? (\sofn{}, \rttc{}) It's unclear how the work's contributions are highlighted in this section. (\rttc{})} Our contribution is to use 3D representations into a diffusion policy. We compare against all prior 3D policies on RLBench under various setups and outperform them by large margins. On CALVIN, we are the first to deploy a 3D policy and the baselines all use 2D representations, as the reviewers correctly state. We show that it can achieve SOTA performance on a benchmark that has been dominated by 2D policies. This is orthogonal to prior works' contributions, such as pre-training on videos (GR-1) and fine-tuning foundation models for action prediction (RoboFlamingo) or subgoal generation (SuSIE), which our model does not employ.

To show that \model{} indeed sets the new state-of-the-art among both 2D and 3D policies, we test another 3D baseline policy--the combination of Act3D and Chained Diffuser--on CALVIN.  Act3D is a strong 3D baseline policy on RLBench, however, the model can only predicts end-effector poses at key frames.  We thus deploy another performant trajectory predictor--Chained Diffuser--to predict intermediate trajectories to reach target poses.  We update the results in Table~\ref{tab:calvin}, showing that this 3D baseline policy significantly underperforms other methods on CALVIN.  The main reason is that Act3D, a deterministic model, fails to learn action prediction from noisy and multimodal play trajectories.

\noindent \textbf{Comparison to GR-1/Was GR-1 also given access to these extra keyposes? (\rttc{})}
Our model is trained to \textbf{predict} keyposes, it is not given access to keyposes at test time. Specifically on CALVIN, our model is trained to jointly predict the next keypose and the trajectory up to that keypose. When deployed, 3D Diffuser Actor simply predicts fixed-length trajectories. We found this temporal abstraction to be useful and more computationally efficient.

We are not the first to use some form of temporal abstraction on CALVIN. For example, HULC++ \cite{mees2023grounding} also uses keyposes, termed \textit{``affordances"} in their paper, although their algorithm for extracting those is different from ours. GR-1 on the other hand experimented with predicting frames that are further away in the future (see Table 5 in their appendix) and found it not to be useful. Reciting GR-1 \textit{``we hypothesize that this is because the model is trained to predict local actions and predicting frames that are too far into the future may not be able to provide good guidance for immediate local action prediction."}

\noindent \textbf{The robustness to noisy calibrations?}
We refer to Table~\ref{tab:noisy_depth} and Section~\ref{sec:noisy_depth} in the Appendix for our evaluation of the robustness to noisy calibrations.

\noindent \textbf{Discussion of failure modes?}  We refer to our Figure~\ref{fig:failure} and Section~\ref{sec:failure} in the Appendix for our discussion of failure modes on RLBench.

==> rss_tex/9_rebuttal_2.tex <==
\clearpage
% \newcommand{\sofn}[1]{{\color{cyan}SoFn}}
% \newcommand{\rttc}[1]{{\color{purple}rTTc}}
% \newcommand{\gyzr}[1]{{\color{blue}GyZr}}

% \input{src/fig_method_comparison}
\noindent \textbf{Comparison to other baseline policies}
We present an overview comparison to Act3D~\cite{gervet2023act3d}, PerAct~\cite{shridhar2023perceiver} and Diffusion Policy~\cite{chi2023diffusion} in Figure~\ref{fig:compare}.  We compare to Act3D and ChainedDiffuser~\cite{xian2023chaineddiffuser} in more details in the following paragraphs.

\noindent \textbf{Ours vs. Act3D}
The main contribution of Act3D is to (1) forego expensive 3D voxelization and (2) preserve equivariance to facilitate generalization in action prediction, by predicting a 3D point action map.  Act3D converts multiview posed RGB-D images into a 3D feature cloud, and encodes language instructions into language tokens.  To obtain a 3D point map, Act3D samples 3D ghost points on a 3D grid, initializes a query token for each sampled points, and features point tokens by cross-attending to the scene 3D feature cloud.  To predict action with the 3D point map, Act3D additionaly initializes a learnable query, that cross-attends to both the 3D feature cloud and language tokens, and scores each sampled point with the similarity of token features.  This process is repeated 3 times, each time with a refined 3D point sampling and more fine-grained visual features to improve map resolution.  At the end, a 3D rotation of the end-effector is regressed from the query features, and a 3D location of the end-effector is derived from the location of the point with the maximal activation.  Act3D is thus a deterministic policy.

The main contribution of \model{} is to (1) forego building 3D point maps and (2) iteratively denoise end-effector poses to handle multimodality in action prediction.  In spite of using the similar scene encoder as Act3D, \model{} considers action prediction as a denoising process conditioned on multiview images and language instructions, instead of a point classification problem.  Our model represents current estimate of the end-effector poses as 3D tokens, that attend to scene 3D feature cloud and language tokens, and outputs the noise in the 3D translation and rotation of the end effector.  To preserve translation invariance, we apply relative attention using relative positions among pose tokens and the scene feature cloud.  \model{} initializes estimate of end-effector poses from pure noise, iterates the denoising process, and at the end, outputs the end-effector poses.

In summary, \model{} differs from Act3D as the former is a diffusion model, iteratively denoising end-effector poses, and the latter is a deterministic model, sampling and scoring 3D points in a fine-to-coarse manner.

\noindent \textbf{Ours vs. ChainedDiffuser}
\model{} is significantly different from ChainedDiffuser.  ChainedDiffuser is a method that combines Act3D and a trajetory diffusion predictor.  The end-effector poses at key frames are predicted deterministically by Act3D.  In contrast, our model is a single diffusion policy that predicts both end-effector poses at key frames and intermediate trajectory to reach end-effector keyposes.

The contribution of ChainedDiffuser is to get rid of sampling-based motion planners, as they fail in tasks that cannot be easily decomposed into straight-line trajectory segments, such as {\it opening doors} or {\it wiping the table}.  It uses trajectory diffusion that conditions on the current and target end-effector poses to predict the intermediate trajectory.

The contribution of \model{} is to propose a single diffusion framework for predicting both (1) end-effector poses at key frames, and (2) the intermediate trajectory to reach target poses.  Our model can thus handle multimodality of action prediction better than ChainedDiffuser.  In fact, to satisfy reviewers' request, we test ChainedDiffuser on CALVIN.  As shown in Table~\ref{tab:calvin}, \model{} is the SOTA policy, while ChainedDiffuser does not work well on CALVIN.


\noindent \textbf{Derivation of 3D scene representation}
We use a 3D scene encoder similar to \cite{gervet2023act3d,xian2023chaineddiffuser}, which extracts 3D scene tokens from posed RGB-D images and gather tokens from multiple camera views into 3D feature cloud.  Our \model{} conditions on the 3D feature cloud and diffuse the trajectory of end-effectory poses.

For camera view $i$, we capture the RGB image $I_{i} \in \mathbb{R}^{H\times W\times 3}$ and the depth map $D_{i} \in \mathbb{R}^{H\times W}$, where $H, W$ denote the height and width in pixels.  To obtain a 3D location map $P_i$, we map each pixel location and depth value to a 3D location in the world frame, using the camera extrinsic/intrinsic parameters and the pinhole camera equation.  To obtain scene features, we encode image $I_i$ to a 2D feature map $F_i \in \mathbb{R}^{\frac{H}{s} \times \frac{W}{s} \times c}$, where $s$ denotes the downsampling ratio of the image encoder and $c$ is the channel dimension.  To obtain 3D scene tokens, we need to map each feature vector in $F_i$ to a 3D location.  We downsample $P_i$ to $P'_i \in \mathbb{R}^{\frac{H}{s} \times \frac{W}{s} \times 3}$ with 2D average pooling, where $P'_i(u, v)$ corresponds to the 3D location of feature vector $F_i(u, v)$ at patch $(u, v)$.  Lastly, we gather 3D scene tokens from multiple camera views into a 3D feature cloud, consisting of token features $\mathbf{F} = \{F_i(u, v) | \forall u, v\}_{i=1}^{N_C}$ and 3D location $\mathbf{P'} = \{P'_i(u,v) | \forall u, v\}_{i=1}^{N_C}$, where $u, v$ denote the row and column index of patch, $i$ is the camera index and $N_C$ is the total number of camera views.  We updated the main paper with this detailed description.


\noindent \textbf{Details of 3D relative position denoising transformer}
We use a 3D relative transformer to diffuse a trajectory of end-effector poses $\mathbf{A} = \{\ac_i\}_{\forall i}$, where $\ac_i = \{\ac^{pos}_i, \ac^{rot}_i, \ac^{open}\}$ denotes the $i^{th}$ pose in the trajectory and $N_T$ is the trajectory length.  At each diffusion step $t$, we represent the estimate of $i^{th}$ pose $\ac_{i,t}$ as a 3D token in the transformer, which attends to 3D scene tokens, all pose estimates $\mathbf{A}_t = \{\ac_{i,t}\}_{\forall i}$, and language instruction tokens to denoise current estimate of the end-effector pose.

In particular, we map the position $\ac^{pos}_{i,t}$ and rotation $\ac^{rot}_{i,t}$ to a pose token $\mathbf{z}_{i,t} \in \mathbb{R}^{F}$ with a MLP, where $\ac^{pos}_{i,t}$ corresponds to the 3D location of $\mathbf{z}_{i,t}$.  We apply cross-/self-attention among all scene tokens $\mathbf{F}$ and pose tokens $Z_t = \{\mathbf{z}_{i,t}\}_{\forall i}$ using their 3D locations $\mathbf{P'}$ and $\mathbf{A}_t^{pos} = \{\ac_{i,t}^{pos}\}_{\forall i}$.  To ensure translation invariance in the denoising transformer, we use the rotary positional embeddings~\cite{su2021roformer} to encode relative positional information in attention layers.  The attention weight between query $q$ and key $k$ is written as: $e_{q, k} \propto \mathbf{x}_q^T \mathbf{M}(\mathbf{p}_q - \mathbf{p}_k) \mathbf{x}_k$, where $\mathbf{x}_q$ / $\mathbf{x}_k$ and $\mathbf{p}_q$ / $\mathbf{p}_k$ denote the features and 3D positions of the query / key, and $\mathbf{M}$ is a matrix function which depends only on the relative positions of the query and key.  We provide a more detailed formulation in Section~\ref{sec:attention} of the Appendix.

For conditioning on language instructions, both scene tokens $\mathbf{F}$ and pose tokens $Z_t$ cross attends to language tokens.  We do not add positional encodings to  $\mathbf{F}$ and $Z_t$, but temporal encodings to the language tokens, which denote the order of each language token in the text.  

Lastly, we use separate MLPs to predict (1) the noise of position, (2) the noise of rotation and (3) the openess of the end-effector, from $Z_t$.  We provide a detailed diagram of our model in Fig.~\ref{fig:detailed_diagram} of the Appendix.

\noindent \textbf{The robustness to noisy calibrations}
\model{} is reasonably robust to noisy calibrations.  We evaluate our model on RLBench with the setup of GNFactor.  We perturb the depth information by adding Gaussian noise to the 3D location of each pixel.  Under mild ($\sigma=0.01$) and strong ($\sigma=0.03$) perturbations, \model{} retains $92\%$ and $64\%$ of the relative performance of that without noise.  Notably, our model has only been trained with perfect calibrations.  We can further enhance the robustness to noisy calibrations by impose corresponding augmentations during training.  We present our experimental results in Table~\ref{tab:noisy_depth} and Section~\ref{sec:noisy_depth} in the Appendix.

\noindent \textbf{Discussion of failure modes}
We discover two major failure modes of \model{}: (1) imprecise action prediction, and (2) confusion of language instruction.  In $50\%$ of the failure cases, it did not predict end-effector poses precisely, and failed to satisfy the success condition.  In $38\%$ of the failure cases, it did not grasp the target object, specified in the language instruction.  In $8\%$ of the failure cases, it failed an intermediate task of a long-horizon task.  In the rest of the failure cases, the motion planner failed to find an optimal path to reach the predicted end-effector pose.  We present the analysis in Figure~\ref{fig:failure} and Section~\ref{sec:failure} in the Appendix.


==> rss_tex/OLD1_abstract.tex <==
\begin{abstract}
We marry  diffusion  policies and 3D scene representations for robot manipulation. 
Diffusion policies learn the action distribution conditioned on the robot and environment state using  conditional diffusion models.  They have recently shown to outperform both deterministic and alternative state-conditioned action distribution learning  methods.  
3D robot policies use 3D scene feature representations aggregated  from a single or multiple camera views using sensed depth. They have shown to  generalize better than their 2D counterparts across camera viewpoints. 
We unify these two lines of work and present \modellong{}, a neural policy architecture 
that, given a language instruction, builds  a 3D  representation of the visual scene  and conditions on it to iteratively denoise 3D rotations and translations for the robot's end-effector.   
At each denoising iteration, our model represents end-effector pose estimates as 3D scene tokens and predicts the 3D translation and rotation error for each of them, by featurizing them using 3D relative attention to other 3D visual and language tokens. 
\modellong{} sets a new state-of-the-art on RLBench with an absolute performance gain of 18.1\%  over the current SOTA on a multi-view setup and an absolute gain of 13.1\% on a single-view setup. 
On the CALVIN benchmark, it outperforms the current SOTA in the setting of zero-shot unseen scene generalization by being able to successfully run \rebut{0.29} more tasks, a \rebut{9\%} relative increase. 
It also works in the real world from a handful of demonstrations. 
We ablate our model's architectural design choices, such as  3D scene featurization  and  
 3D relative  attentions, and show they all help generalization. 
Our results suggest that 3D scene representations and powerful generative modeling are keys to efficient robot learning from demonstrations.  
\end{abstract}




==> rss_tex/OLD2_introduction.tex <==
\section{Introduction}
\label{sec:intro}

Many robot manipulation tasks 
are inherently multimodal: at any point during task execution, there may be multiple actions which yield task-optimal behavior. Indeed, human demonstrations often contain diverse ways that a task can be accomplished. 
A natural choice  is then to treat policy learning as a distribution learning problem: instead of representing a policy as a deterministic map $\pi_\theta(x)$,  learn the entire distribution of actions conditioned on the current robot state $p(y|x)$ \cite{DBLP:journals/corr/HoE16,tsurumine2022goalaware,DBLP:journals/corr/HausmanCSSL17,shafiullah2022behavior}. 



\HL{Recent works  use diffusion policies for learning such state-conditioned action distributions for robot manipulation policies from demonstrations }\cite{pearce2023imitating,chi2023diffusion,reuss2023goal}. 
They show they outperform  deterministic or other  alternatives, such as variational autoencoders \cite{IRIS}, mixture of Gaussians \cite{10.1145/1329125.1329407}, combination of classification and regression objectives \cite{shafiullah2022behavior}, or energy-based objectives \cite{DBLP:journals/corr/abs-2109-00137}. %Specifically, they exhibit better action distribution coverage and higher fidelity (less mode hallucination) than alternative formulations \cite{pearce2023imitating}.  
They have so far been used with either low-dimensional engineered state representations \cite{pearce2023imitating} or 2D  image representations  \cite{chi2023diffusion}.

\begin{comment}

\input{src/fig_teaser}
\end{comment}
% \begin{figure*}[h!]
%     \centering
%     \begin{adjustbox}{center}
%     \includegraphics[width=1.0\textwidth,keepaspectratio]{figs/teaser.pdf}
%     \end{adjustbox}    
%     \caption{{\textbf \model{}} is a language and vision conditioned action diffusion policy that learns to predict end-effector keyposes and trajectories from demonstrations.  (a) An image encoder  extracts a 2D image feature map from each camera view;  each feature token corresponds to a fixed-size patch in the input image. 
%     (b) We lift  2D feature tokens to 3D using sensed depth.  \rebut{(c) We encode language instructions with a pre-trained language encoder.  (d)} A 3D relative position attention Transformer  takes as input   the 3D scene tokens, an instruction text encoding,  a short history of  end-effector poses and the current noisy estimate of the end-effector future trajectory (or keypose) and outputs the noise in the form of 3D translations and rotations.
%     }
%     \label{fig:overview}
% \end{figure*}

\HL{Many recent research works have pursued bird's eye view or 3D scene representations for learning robot policies from demonstrations}, such as Transporter Networks  \cite{zeng2021transporter,huang2024fourier}, C2F-ARM~\cite{james2022coarse},  PerAct~\cite{shridhar2023perceiver}, Act3D \cite{gervet2023act3d} and Robot View Transformer \cite{goyal2023rvt}. 
They ``lift" features from perspective views to a bird's eye view (BEV) or 3D  robot workspace, and  have  shown strong  empirical results %in robot learning from demonstrations
\cite{shridhar2023perceiver, james2022coarse, goyal2023rvt, gervet2023act3d}. 
Specifically, such 3D policy formulations  have shown to 
%Policies that use such 2D-to-BEV or 2D-to-3D scene encodings
generalize better than  2D robot policies across camera viewpoints and  to handle   novel camera viewpoints at test time \cite{gervet2023act3d,goyal2023rvt}. We conjecture this improved performance comes from the fact that the 3D visual scene tokens and the robot's end-effector interact in a common 3D space. 
3D policy formulations handle action multimodality by discretizing the robot's  workspace  in order to predict the future 3D location of  the robot's end-effector, such as the 2D BEV map for pick and place actions \cite{zeng2021transporter}, the 3D workspace \cite{gervet2023act3d}, or multiview re-projected images \cite{goyal2023rvt}. 
 3D robot policies have not yet been combined yet with diffusion objectives.
 \HL{  ChainedDiffuser \cite{xian2023chaineddiffuser} uses a diffusion model that takes as input 3D end-effector keyposes predicted by Act3D \cite{gervet2023act3d} and a 3D representation of the scene to infer end-effector 3D trajectories that link the current end-effector pose to the predicted one. ChainedDiffuser  uses diffusion models as a drop-in replacement for motion planners, rather than  manipulation policies, since it relies on Act3D, which is a deterministic model, for 3D keypose prediction. We compare against ChainedDiffuser in our experiments and show we greatly outperform it.}

In this paper, we propose \modellong{}, a model that marries  diffusion policies for handling action multimodality and 3D scene encodings for effective spatial reasoning. \modellong{} trains a  denoising neural network 
that takes as input a 3D scene visual encoding, the current estimate of the end-effector's  future trajectory (3D location and orientation), as well as the noise level index, and  predicts the error in 3D translation and rotation. 
Our model achieves translation equivariance in prediction by representing the current estimate of the robot's end-effector trajectory as 3D scene tokens and featurizing them jointly with the visual tokens using relative-position 3D attentions \cite{shaw2018selfattention,su2021roformer}.%, as shown in Figure \ref{fig:overview}. 



We test \modellong{} in  learning robot manipulation policies from demonstrations on the simulation benchmarks of RLBench \cite{james2020rlbench} and CALVIN \cite{mees2022calvin}, as well as in the real world. Our model sets a new state-of-the-art on RLBench, outperforming existing 3D policies and 2D diffusion policies with a 18.1\% absolute gain on multi-view setups and 13.1\% on single-view setups (Figure~\ref{fig:teaser}). On CALVIN, our model outperforms the current SOTA in the setting of zero-shot unseen scene generalization by a \rebut{9\%} relative gain (Figure~\ref{fig:teaser}). 
We additionally show that \modellong{} outperforms all existing policy formulations that either do not use 3D scene representations or do not use action diffusion, as well as  ablative versions of our model that do not use 3D relative attentions. 
We further show \modellong{} can learn multi-task manipulation in the real world across 12 tasks from a handful of real-world demonstrations. Simulation and real-world robot execution videos are included as part of our supplementary material. 
%Simulation and real-world robot execution videos, as well as our code and trained checkpoints are publicly available on our website: \url{3d-diffuser-actor.github.io}.

\HL{In summary, our  contributions are as follows:
\begin{enumerate}
\item  Combining 3D scene representations with diffusion objectives for learning robot policies. 
\item State-of-the-art performance in established benchmarks, much above previous works.
\end{enumerate}
}
Our models and code will be publicly available upon publication.




==> rss_tex/OLD3_relatedwork.tex <==
\section{Related Work}
\label{sec:work}

\input{src/fig_method_comparison}

\noindent \textbf{Learning robot manipulation policies from demonstrations}

Though state-to-action mappings are typically multimodal, earlier works on learning from demonstrations train deterministic policies with behavior cloning \cite{Pomerleau-1989-15721,DBLP:journals/corr/BojarskiTDFFGJM16}. 
To better handle action multimodality, other approaches  discretize action dimensions  and use cross entropy losses \cite{semanetlang,shridhar2023perceiver,zeng2021transporter}.  
However, the number of bins needed to approximate a continuous action space grows exponentially with increasing dimensionality. 
Generative adversarial networks \cite{DBLP:journals/corr/HoE16,tsurumine2022goalaware,NEURIPS2019_c8d3a760}, variational autoencoders \cite{IRIS} and combined Categorical and Gaussian distributions \cite{shafiullah2022behavior,guhur2023instruction,Cui2022FromPT} have been used to learn from multimodal demonstrations. 
Nevertheless, these models tend to be sensitive to hyperparameters, such as the number of clusters used \cite{shafiullah2022behavior}.
Implicit behaviour cloning  represents distributions over actions by using Energy-Based Models (EBMs) \cite{DBLP:journals/corr/abs-2109-00137,ta2022conditional}. Optimization in EBMs amounts to searching the energy landscape for minimal-energy action, given a state. EBMs are inherently multimodal, since the learned landscape can have more than one minima. EBMs are also composable, which makes them suitable for combining action distributions with additional constraints during inference \cite{gkanatsios2023energy}. Diffusion models \cite{sohldickstein2015deep,DDPM} are a powerful class of generative models related to EBMs in that they   model the score of the  distribution, else, the gradient of the energy, as opposed to the energy itself \cite{singh2023revisiting,salimans2021should}. The key idea behind diffusion models is to iteratively transform a simple prior distribution into a target distribution by applying a sequential denoising process. They have been used for modeling state-conditioned action distributions in imitation learning \cite{ryu2023diffusion,urain2023se,pearce2023imitating,wang2022diffusion,reuss2023goal,mishra2023reorientdiff}  from low-dimensional input, as well as from visual sensory input,
and show both better mode coverage and higher fidelity in action prediction than alternatives. They have not been yet combined with 3D scene representations.


\noindent\textbf{Diffusion models in robotics}
Beyond policy representations in imitation learning, diffusion models have been used to model cross-object and object-part arrangements \cite{liu2022structdiffusion,simeonov2023shelving,mishra2023reorientdiff,fang2023dimsam,gkanatsios2023energy} and visual image subgoals \cite{kapelyukh2023dall,dai2023learning,ajay2023hip,black2023zero}. They have also been used successfully in offline reinforcement learning \cite{chen2023offline,yang2024diffusiones,hansen2023idql}, where they model the state-conditioned action trajectory distribution \cite{hansen2023idql,chen2023offline} or state-action trajectory distribution \cite{janner2022planning, he2023diffusion, Wang2023ColdDO}. ChainedDiffuser~\cite{xian2023chaineddiffuser} 
proposes to replace motion planners, commonly used for  keypose  to keypose linking, with a trajectory diffusion model that conditions on the 3D scene feature cloud and the predicted target 3D keypose to denoise a trajectory from the current to the target keypose. 3D Diffuser Actor instead predicts the next 3D keypose for the robot's end-effector alongside the linking trajectory, which is a much harder task than linking two given keyposes. 
Lastly, image diffusion models have  been used for augmenting the conditioning  images input to robot policies to help the latter generalize better \cite{liang2023adaptdiffuser,chen2023genaug,mandi2022cacti}.


\noindent\textbf{2D and 3D scene representations for robot  manipulation} 
End-to-end image-to-action policy models, such as RT-1~\cite{brohan2022rt}, RT-2~\cite{brohan2023rt2}, GATO~\cite{reed2022generalist}, BC-Z~\cite{jang2022bc}, RT-X~\cite{Padalkar2023OpenXR}, Octo~\cite{octo_2023} and InstructRL~\cite{liu2022instruction} leverage transformer architectures for the direct prediction of 6-DoF end-effector poses from 2D video input. However, this approach comes at the cost of requiring thousands of demonstrations to implicitly model 3D geometry and adapt to variations in the training domains. Another line of research is centered around Transporter networks \cite{zeng2021transporter,seita2021learning,shridhar2022cliport, gkanatsios2023energy}, demonstrating remarkable few-shot generalization by framing end-effector pose prediction as pixel classification. Nevertheless, these models are usually confined to top-down 2D planar environments with simple pick-and-place primitives. Direct extensions to 3D, exemplified by C2F-ARM~\cite{james2022coarse} and PerAct~\cite{shridhar2023perceiver}, involve voxelizing the robot's workspace and learning to identify the 3D voxel containing the next end-effector keypose \HL{(Figure~\ref{fig:compare})}. However, this becomes computationally expensive as resolution requirements increase. Consequently, related approaches resort to either coarse-to-fine voxelization, equivariant networks \cite{huang2024fourier} or efficient attention operations~\cite{jaegle2021perceiver} to mitigate computational costs.
Act3D \cite{gervet2023act3d} foregoes 3D scene voxelization altogether; it instead computes a 3D action map of  variable spatial resolution by sampling 3D points in the empty workspace and featurizing them using cross-attentions to the  3D physical points. Robotic View Transformer (RVT) \cite{goyal2023rvt} re-projects the input RGB-D image to alternative image views, featurizes those and lifts the predictions to 3D to infer 3D locations for the robot's end-effector. \HL{\model{} adopts the scene encoder of Act3D but is a probabilistic diffusion model, iteratively denoising end-effector poses. We highlight the differences between our model and other related works in Figure~\ref{fig:compare}. Act3D is a deterministic model, sampling and scoring 3D points in a coarse-to-fine manner to predict 3D locations and regress 3D orientations. \model{} foregoes predicting 3D action maps altogether and considers action prediction as a denoising process conditioned on  images and language instructions, instead of a point classification problem. We refer to Figures \ref{fig:detailed_diagram}, \ref{fig:act3d_detailed_diagram} in the Appendix for more details on the technical differences between Act3D and \model{}.} %Both Act3D and RVT show currently the highest performance on RLBench \cite{james2020rlbench}.
Our model outperforms Act3D and RVT by a big margin, as we show in the experimental section.


\noindent \textbf{Instruction-conditioned long-horizon policies}
To generate actions based on language instructions, early works~\cite{lynch2020language,mees2022hulc,brohan2022rt} employ a text encoder to map language instructions to latent features,  then they deploy 2D policies that condition on these language latents to predict actions. HULC++ \cite{mees2023grounding} alternates between a free-space policy that reaches subgoals (next object to interact with) and a local policy \cite{mees2022hulc} for low-level interaction. However, these models struggle to infer 3D actions precisely from 2D observations and language instructions and do not generalize to new environments with different texture.  Recent works~\cite{black2023zero,li2023vision,wu2023unleashing} explore the use of large-scale pre-training to boost their performance. SuSIE~\cite{black2023zero} proposes to synthesize visual subgoals using InstructPix2Pix~\cite{brooks2023instructpix2pix}, an instruction-conditioned image generative model pre-trained on a subset of 5 billion images~\cite{schuhmann2022laion}.  Actions are then predicted by a low-level diffusion policy conditioned on both current observations and synthesized visual goals.  RoboFlamingo~\cite{li2023vision} fine-tunes existing vision-language models, pre-trained for solving vision and language tasks, to predict the robot's actions.  GR-1~\cite{wu2023unleashing} pre-trains a GPT-style transformer for video generation on a massive video corpus, then jointly trains the model for predicting robot actions and future observations. We show that \model{} can exceed the performance of these policies thanks to effective use of 3D representations.

==> rss_tex/OLD4_method.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{src/fig_arch}
% \figArchitecture{htb}


\section{Method}
\label{sec:method}


The architecture of \model{} is shown in Figure~\ref{fig:architecture}. 
It is a conditional  diffusion  model that takes as input  visual observations, a language instruction, the robot's end-effector's current pose \rebut{(proprioceptive information)} and the current estimate for the robot's future action trajectory, and predicts the error in the end-effector's 3D translations and 3D orientations for each predicted timestep. 
We review  Denoising Diffusion Probabilistic models  in Section \ref{subsec:diffusion_prelim} and  describe the architecture and training details of our model in Section \ref{subsec:architecture}.



\subsection{\model{}}
\label{subsec:architecture}
We next describe the architecture of our model that predicts the end-effector's trajectory error given the current noisy estimate, a visual scene encoding, a language instruction, the denoising iteration index and the end-effector's \rebut{proprioceptive information}. % \rebut{We present an overview comparison to other methods other baselines, such as Act3D~\cite{gervet2023act3d}, PerAct~\cite{shridhar2023perceiver} and Diffusion Policy~\cite{chi2023diffusion} in Figure~\ref{fig:compare}.}

\noindent \textbf{Observation space and action representation} 3D Diffuser Actor is trained on demonstrations of successful trajectories in the form of $\{(o_1, \ac_1), (o_2, \ac_2), ...\}$, accompanied with a task language description, similar to previous works \cite{james2022q, shridhar2023perceiver, gervet2023act3d, wu2023unleashing}. Each observation $o$ comprises a set of posed  (multi-view) RGB-D images. 
Each action $\ac$ describes an end-effector pose and is decomposed into 3D position, 3D orientation and a binary open/closed state: 
$\ac = \{ \ac^{\mathrm{\small pos}} \in \mathbb{R}^3, \ac^{\mathrm{\small rot}} \in \mathbb{R}^6, \ac^{\mathrm{\small open}} \in \{0,1\}\} $. We represent rotations using the  6D rotation representation
of \cite{zhou2020continuity} for all environments in all our experiments, to avoid the discontinuities of the quaternion representation. 

\noindent \textbf{Keyposes} \model{} inherits the temporal abstraction of demonstrations into end-effector \textit{keyposes} from previous works \cite{james2022q, shridhar2023perceiver, gervet2023act3d, liu2022instruction}. Keyposes are important intermediate end-effector poses that summarize a demonstration and can be extracted using simple heuristics, such as a change in the open/close end-effector state or local extrema of velocity/acceleration. We describe the heuristics we use for each dataset in the Appendix (Section~\ref{sec:heuristics_calvin}). During inference, \model{} can either predict and execute the full trajectory of actions up to the next keypose (including the keypose), or just predict the next keypose and use a sampling-based motion planner to reach it, similar to previous works \cite{shridhar2023perceiver,guhur2023instruction,gervet2023act3d}. In the rest of this section we use the term ``trajectory" to refer to \model{}'s output. Keypose prediction is a special case where the trajectory contains  only one future pose. 

\noindent \textbf{Scene and language encoder} 
We use a scene and language encoder similar to \cite{gervet2023act3d,xian2023chaineddiffuser}, which extract 3D scene tokens from posed RGB-D images and gather tokens from multiple camera views into 3D feature cloud. We describe it here to make the paper self-contained. \HL{For each camera view $i$, we capture the RGB image $I_{i} \in \mathbb{R}^{H\times W\times 3}$ and the depth map $D_{i} \in \mathbb{R}^{H\times W}$, where $H, W$ denote the height and width in pixels. We obtain a 3D location map $P_i \in \mathbb{R}^{H\times W\times 3}$ by mapping each pixel location and depth value to a 3D location in the world frame, using the camera extrinsic/intrinsic parameters and the pinhole camera equation. We obtain scene features by encoding each image $I_i$ to a 2D feature map $F_i \in \mathbb{R}^{\frac{H}{s} \times \frac{W}{s} \times d}$, where $s$ denotes the downsampling ratio of the image encoder and $d$ is the channel dimension. To obtain the 3D scene tokens, we need to map each feature vector in $F_i$ to a 3D location.  We downsample $P_i$ to $P'_i \in \mathbb{R}^{\frac{H}{s} \times \frac{W}{s} \times 3}$ with 2D average pooling, where $P'_i(u, v)$ corresponds to the 3D location of feature vector $F_i(u, v)$ at patch $(u, v)$.  Lastly, we gather 3D scene tokens from multiple camera views into a 3D feature cloud, consisting of token features $\mathbf{F} = \{F_i(u, v) | \forall u, v\}_{i=1}^{N_C}$ and 3D location $\mathbf{P'} = \{P'_i(u,v) | \forall u, v\}_{i=1}^{N_C}$, where $u, v$ denote the row and column index of patch, $i$ is the camera index and $N_C$ is the total number of camera views.}

The language encoder maps language task descriptions or instructions into language feature tokens. We use the pre-trained CLIP ResNet50 2D image encoder ~\cite{radford2021learning} to encode each RGB image into a 2D feature map and the pre-trained CLIP language encoder to featurize the  language task instruction.




\noindent\textbf{3D Relative Position Denoising Transformer}
\rebut{We use a 3D relative transformer to diffuse a trajectory of end-effector poses $\mathbf{A} = \{\ac_j\}_{\forall j}$, where $\ac_j = \{\ac^{pos}_j, \ac^{rot}_j, \ac_j^{open}\}$ denotes the $j^{th}$ pose in the trajectory.  At each diffusion step $t$, we represent the estimate of $j^{th}$ pose $\ac_{j,t}$ as a 3D token in the transformer, which attends to 3D scene tokens, all pose estimates $\mathbf{A}_t = \{\ac_{j,t}\}_{\forall j}$, and language instruction tokens to denoise current estimate of the end-effector pose.

In particular, we map the position $\ac^{pos}_{j,t}$ and rotation $\ac^{rot}_{j,t}$ to a pose token with a MLP, where $\ac^{pos}_{j,t}$ corresponds to the 3D location of the pose token.  We apply cross-/self-attention among all scene tokens $\mathbf{F}$ and all pose tokens using their 3D locations $\mathbf{P'}$ and $\mathbf{A}_t^{pos} = \{\ac_{j,t}^{pos}\}_{\forall j}$.  To ensure translation invariance in the denoising transformer, we use the rotary positional embeddings~\cite{su2021roformer} to encode relative positional information in attention layers, inspired by recent work in visual correspondence \cite{Li2021LepardLP,Gkanatsios2023AnalogyFormingTF} and 3D manipulation \cite{gervet2023act3d,xian2023chaineddiffuser}.  The attention weight between query $q$ and key $k$ is written as: $e_{q, k} \propto \mathbf{x}_q^T \mathbf{M}(\mathbf{p}_q - \mathbf{p}_k) \mathbf{x}_k$, where $\mathbf{x}_q$ / $\mathbf{x}_k$ and $\mathbf{p}_q$ / $\mathbf{p}_k$ denote the features and 3D positions of the query / key, and $\mathbf{M}$ is a matrix function which depends only on the relative positions of the query and key.  We provide a more detailed formulation in Section~\ref{sec:attention} of the Appendix.

% For conditioning on language instructions, both scene tokens $\mathbf{F}$ and pose tokens $Z_t$ cross attends to language tokens.  We do not add positional encodings to  $\mathbf{F}$ and $Z_t$, but temporal encodings to the language tokens, which denote the order of each language token in the text.  

Lastly, we use separate MLPs to predict (1) the noise of position $\epsilon_\theta^{\mathrm{\small pos}}(o, l, c,\mathbf{A}_{\id}^{\mathrm{\small pos}}, \mathbf{A}_{\id}^{\mathrm{\small rot}},\id)$, (2) the noise of rotation $\epsilon_\theta^{\mathrm{\small rot}}(o, l, c, \mathbf{A}_{\id}^{\mathrm{\small pos}},\mathbf{A}_{\id}^{\mathrm{\small rot}},\id)$ and (3) the openess of the end-effector $f_\theta^{\mathrm{\small open}}(o,l,c,\mathbf{A}_{\id}^{\mathrm{\small pos}},\mathbf{A}_{\id}^{\mathrm{\small rot}},\id)$, from pose tokens.  Here, $o$ denotes the visual observations, $l$ the input language and $c$ the proprioception information.
}
% 3D Diffuser Actor iteratively denoises an estimate of the end-effector's future trajectory. Every trajectory step token is a 10-dimensional action, as defined earlier. We map each such action into a high-dimensional representation through an MLP \color{orange}to obtain a trajectory representation $Z_T \in \mathbb{R}^{N_T \times F}$, with $N_T$ the number of trajectory tokens\color{black}. Each action token comes with the positional embeddings of its corresponding $\ac^{\mathrm{\small pos}}$. 
% We incorporate proprioceptive information as a short, \HL{fixed-length} history of predicted end-effector keyposes. These are represented with learnable feature vectors $Z_c \in \mathbb{R}^{N_h \times F}$, where $N_h$ the history length, and their 3D positions are used to compute positional embeddings. \rebut{probably remove $Z_c$?}

% We contextualize all tokens, namely visual $o$, language $l$, proprioception $c$ and action tokens (current estimate) $\ac_t^{pos}, \ac_t^{rot}$
% We contextualize all tokens, namely visual $Z_o$, language $Z_l$, proprioception $Z_c$ and action tokens (current estimate) $Z_T$ using 3D relative position attention layers. \color{orange}Specifically, the scene tokens $Z_o$ first attend to the language tokens $Z_l$. Then, the trajectory tokens $Z_T$ attend to the updated scene tokens $Z'_o$. Lastly, we concatenate the updated trajectory $Z'_T$ and scene tokens $Z'_o$ along the sequence dimension and feed to self-attention layers. The proprioception tokens and the denoising step are used as conditional inputs to every attention layer in the model using the FiLM technique \cite{perez2018film}. \color{black}  
% Inspired by recent work in visual correspondence \cite{Li2021LepardLP,Gkanatsios2023AnalogyFormingTF} and 3D manipulation \cite{gervet2023act3d,xian2023chaineddiffuser}, we use rotary positional embeddings \cite{su2021roformer} with the property that the dot product of two positionally encoded features $\mathbf{x}_i, \mathbf{x}_j$ is:
% \begin{align}
% \mathbf{PE}(\mathbf{p}_i, \mathbf{x}_i)^T \mathbf{PE}(\mathbf{p}_j, \mathbf{x}_j)
%      = \mathbf{x}_i^T \mathbf{M}(\mathbf{p}_j - \mathbf{p}_i) \mathbf{x}_j
% \end{align}
% where $\mathbf{M}$ is a matrix function which depends only on the relative positions of points $\mathbf{p}_i$ and $\mathbf{p}_j$ and thus is translation-invariant.  \rebut{The detailed formulation of attention is shown in the Appendix (Section~\ref{sec:attention}).}

% The updated action feature tokens are fed to MLPs to predict the position error $\epsilon_\theta^{\mathrm{\small pos}}(o, l, c,\ac_{\id}^{\mathrm{\small pos}},\ac_{\id}^{\mathrm{\small rot}},\id)$, rotation error $\epsilon_\theta^{\mathrm{\small rot}}(o, l, c,\ac_{\id}^{\mathrm{\small pos}},\ac_{\id}^{\mathrm{\small rot}},\id)$ and whether the end-effector should be open or closed $f_\theta^{\mathrm{\small open}}(o,l,c,\ac_{\id}^{\mathrm{\small pos}},\ac_{\id}^{\mathrm{\small rot}},\id)$. Here, $o$ denotes the visual observations, $l$ the input language, $c$ the proprioception information and  $\ac_t^{pos}, \ac_t^{rot}$ the action tokens (current estimate).
We use a modified version of Equation \ref{eq:diffupdate} to update the current estimate of each element of the end-effector's trajectory:
\rebut{
\begin{align}
\mathbf{A}^{\mathrm{\small pos}}_{\id-1} = & \frac{1}{\sqrt{\alpha_{\id}}} \left( \mathbf{A}^{\mathrm{\small pos}}_\id - \frac{\beta_\id}{\sqrt{1-\bar{\alpha}_\id}} \epsilon_\theta^{\mathrm{\small pos}}(o,l,c,\mathbf{A}_{\id}^{\mathrm{\small pos}},\mathbf{A}_{\id}^{\mathrm{\small rot}},\id) \right) \nonumber\\
&+\frac{1 - \bar{\alpha}_{\id+1}}{1 - \bar{\alpha}_{\id}}\beta_{\id} \mathbf{z}^{\small pos} \\
\mathbf{A}^{\mathrm{\small rot}}_{\id-1} = &\frac{1}{\sqrt{\alpha_{\id}}} \left( \mathbf{A}^{\mathrm{\small rot}}_\id - \frac{\beta_\id}{\sqrt{1-\bar{\alpha}_\id}} \epsilon_\theta^{\mathrm{\small rot}}(o,l,c,\mathbf{A}_{\id}^{\mathrm{\small rot}},\mathbf{A}_{\id}^{\mathrm{\small rot}},\id) \right) \nonumber\\
&+\frac{1 - \bar{\alpha}_{\id+1}}{1 - \bar{\alpha}_{\id}}\beta_{\id} \mathbf{z}^{\small rot}
\end{align}
}
where $\mathbf{z}^{\small pos},\mathbf{z}^{\small rot}\sim \mathcal{N} (\bzero,\bone) $ variables of appropriate dimension.

We use the following two noise schedulers:
\begin{enumerate}
    \item a scaled-linear noise scheduler $\beta_\id = (\beta_{\max} - \beta_{\min})\id + \beta_{\min}$, where $\beta_{\max}, \beta_{\min}$ are hyperparameters, set to $0.02$ and $0.0001$ in our experiments,
    \item a squared cosine noise scheduler
    $\beta_\id = \frac{1 - \cos\big(\frac{(\id+1)/\maxid + 0.008}{1.008} * \frac{\pi}{2}\big)^2}{\cos\big(\frac{\id/\maxid + 0.008}{1.008} * \frac{\pi}{2}\big)^2}$.
\end{enumerate}
We found using a scaled-linear noise scheduler for denoising end-effector's 3D positions  and a squared cosine noise scheduler for denoising the end-effector's 3D orientations to converge much faster than using squared cosine noise for both.


\noindent \textbf{Training}
\model{} is trained on a dataset of kinesthetic demonstrations, which consists of tuples of RGB-D observations, proprioception information of robot's end-effector pose $c$, action trajectories $\mathbf{A}=[\mathbf{A}^{pos}, \mathbf{A}^{rot}, \mathbf{A}^{open}]$ and corresponding language goals $\{(o_1, c_1, \mathbf{A}_1, l_1),(o_2, c_2, \mathbf{A}_2, l_2), ...\}$.  During training, we randomly sample a diffusion step $\id$ and add noise $\epsilon = (\epsilon^{\mathrm{\small pos}}_\id, \epsilon^{\mathrm{\small rot}}_\id)$ to the ground-truth target poses (position and rotation).  We supervise \model{} using a denoising objective: conditioning on the tuple of $(o, l, c, t)$, our model learns to reconstruct the clean actions by predicting the pose transformation with respect to the current estimate.  We use the $L1$ loss for reconstructing the 3D position and 3D rotation error. We use binary cross-entropy loss to supervise end-effector opening $f_\theta^{\mathrm{\small open}}$. Our objective reformulates Equation~\ref{e:diffloss} into:

\rebut{
\begin{align}
    \mathcal{L}_\theta =& \mathrm{BCE}(f_\theta^{\mathrm{\small open}}(    o, l, c,\mathbf{A}_{\id}^{\mathrm{\small pos}},\mathbf{A}_{\id}^{\mathrm{\small rot}},\id),\mathbf{A}^{\mathrm{\small open}}) \nonumber \\
    &+ w_1 \cdot \|(\epsilon_\theta^{\mathrm{\small pos}}(o, l, c,\mathbf{A}_{\id}^{\mathrm{\small pos}},\mathbf{A}_{\id}^{\mathrm{\small rot}},\id) - \epsilon_{\id}^{\mathrm{\small pos}}\| \nonumber\\
    &+ w_2 \cdot \|(\epsilon_\theta^{\mathrm{\small rot}}(o, l, c,\mathbf{A}_{\id}^{\mathrm{\small pos}},\mathbf{A}_{\id}^{\mathrm{\small rot}},\id) - \epsilon^{\mathrm{\small rot}}_\id \| ,
\end{align}
}
where $w_1,w_2$ are hyperparameters estimated using cross-validation. 

\noindent \textbf{Implementation details} 
We augment RGB-D observations with random rescaling and cropping.  Nearest neighbor interpolation is used for rescaling RGB-D observations. 
To reduce the memory footprint in our 3D Relative Transformer, we use Farthest Point Sampling to sample a subset of the points in the input 3D feature cloud.  We use FiLM~\cite{perez2018film} to inject conditional input, including the diffusion step and proprioception, to every attention layer in the model. We include a detailed architecture diagram of our model and a table of hyper-parameters used in our experiments in the Appendix (Section~\ref{sec:details} and Section~\ref{sec:hyper_parameter}). 


==> rss_tex/OLD5_exps_2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experiments}
\label{sec:experiment}

We test \model{} in learning multi-task manipulation policies on RLBench \cite{james2020rlbench} and CALVIN \cite{mees2022calvin}, two established learning from demonstrations benchmarks. We compare against the current state-of-the-art on single-view and multi-view setups, as well as against ablative versions of our model that do not consider 3D scene representations or relative attention. We also test \model{}'s ability to learn multi-task policies from real-world demonstrations. 


% \input{src/fig_task.tex}


\subsection{Evaluation on RLBench}
\noindent \textbf{Setup}
RLBench is built atop the CoppelaSim~\cite{rohmer2013v} simulator, where a Franka Panda Robot is used to manipulate the scene. 
Our \model{} is trained to predict the next end-effector keypose and we employ the low-level motion planner BiRRT~\cite{kuffner2000rrt}, native to RLBench, to reach the predicted pose, following previous works~\cite{shridhar2023perceiver,gervet2023act3d}. Our model does not perform collision checking for our experiments. We train and evaluate \model{} on two experimental setups of multi-task manipulation:
\begin{enumerate}
    \item \textit{PerAct setup} introduced in \cite{shridhar2023perceiver}:  This uses a suite of 18 manipulation tasks, each task has 2-60 variations, which concern scene variability across object poses, appearance and semantics. The tasks are specified by language descriptions. There are  four cameras available (front, wrist, left shoulder, right shoulder). 
    There are 100 training demonstrations available per task, evenly split across task variations and 25 unseen test episodes for each task. Due to the randomness of the sampling-based motion planner, we test our model across 5 random seeds. During evaluation, models are allowed to predict a maximum of 25 keyposes, unless they receive earlier task-completion indicators from the simulation environment.

    \item \textit{GNFactor setup} introduced in \cite{ze2023gnfactor}: 
    This uses a suite of 10 manipulation tasks (a subset of PerAct's task set). Only one RGB-D camera view is available  (front camera).  There are 20 training demonstrations per task, evenly split across variations.
    %We follow the multi-tasking setup of GNFactor~\cite{ze2023gnfactor} and test \model{}'s ability to operate under a single camera RGB-D view (front camera). Following~\cite{ze2023gnfactor}, we test on a subset of 10 tasks from PerAct.  We train our model using 20 demonstrations per task, evenly split across variations. 
    The evaluation setup mirrors that of PerAct, with the exception that we test the final checkpoint using 3, rather than 5, random seeds on the test set.
\end{enumerate}


\noindent \textbf{Baselines} 
We consider the following baselines:
\begin{enumerate}
    \item C2F-ARM-BC~\cite{james2022coarse}, a 3D policy that iteratively voxelizes RGB-D images and predicts actions in a coarse-to-fine manner. Q-values are estimated within each voxel and the translation action is determined by the centroid of the voxel with the maximal Q-values. 

    \item PerAct~\cite{shridhar2023perceiver},  a 3D policy that voxelizes the workspace and detects the next voxel action through global self-attention.  

    \item Hiveformer~\cite{guhur2023instruction}, a 3D policy that enables attention between features of different history time steps. 

    \item PolarNet~\cite{Chen2023PolarNet3P}, a 3D policy that computes dense point representations for the robot workspace using a PointNext backbone \cite{Qian2022PointNeXtRP}. 

    \item RVT~\cite{goyal2023rvt}, a 3D policy that deploys a multi-view transformer to predict actions and fuses those across views by back-projecting to 3D. 

    \item Act3D ~\cite{gervet2023act3d}, a 3D policy that featurizes the robot's 3D workspace using coarse-to-fine sampling and featurization. 
%\textbf{5.} InstructRL~\cite{liu2022instruction}, a 2D policy that directly predicts 6 DoF poses from image and language conditioning with a pre-trained vision-and-language backbone.

    \item GNFactor~\cite{ze2023gnfactor}, a 3D policy that co-optimizes a neural field for reconstructing the 3D voxels of the input scene and a PerAct module for predicting actions based on voxel representations.
\end{enumerate}


We report results for RVT, PolarNet and GNFactor based on their respective papers. Results for CF2-ARM-BC and PerAct are presented as reported in RVT~\cite{goyal2023rvt}. Results for Hiveformer are copied from PolarNet~\cite{Chen2023PolarNet3P}.

We observed that Act3D~\cite{gervet2023act3d} does not follow the same setup as PerAct on RLBench. Specifically, Act3D uses different 1) 3D object models, 2) success conditions, 3) training/test episodes and 4) maximum numbers of keyposes during evaluation.  For fair comparison, we retrain and test Act3D on the same setup.

We also compare to the following ablative versions of our model:
\begin{enumerate}
    \item \textit{2D Diffuser Actor}, our implementation of  \cite{chi2023diffusion}.  We remove the 3D scene encoding from \model{} and instead  use per-image 2D representations by average-pooling features within each view.  We  add learnable embeddings to distinguish between different views.  We use standard attention layers for joint encoding the action estimate and 2D image features.
    
    \item \textit{\model{} w/o Rel. Attn.}, an ablative version of our model that uses standard (non-relative) attentions to featurize the current  rotation and translation estimate with the 3D scene feature cloud. This version of our model is not translation-equivariant.
\end{enumerate}


\noindent \textbf{Evaluation metrics} 
Following previous work \cite{gervet2023act3d,shridhar2023perceiver}, we evaluate policies by task completion success rate, which is the proportion of execution trajectories that achieve the goal conditions specified in the language instructions.


\input{src/tab_peract}
\noindent \textbf{Results on the  PerAct setup} 
We show quantitative results in Table~\ref{tab:peract}. Our \model{} outperforms all baselines on most tasks by a large margin. It achieves an average $81.3\%$ success rate among all 18 tasks, an absolute improvement of $+18.1\%$ over Act3D, the previous state-of-the-art.  In particular, \model{} achieves big leaps on tasks with multiple modes, such as {\it stack blocks}, {\it stack cups} and {\it place cups}, which most baselines fail to complete. We obtain substantial improvements of $+39.5\%$, $+18.4\%$, $+41.6\%$ and $+20.8\%$ on {\it stack blocks}, {\it put in cupboard}, {\it insert peg} and {\it stack cups} respectively.  %Notably, the original success condition for the {\it close jar} task, as defined by PerAct's RLBench library, is incorrect, leading to failure in all expert demonstrations. We report our results using the corrected success condition proposed in this pull request\footnote{https://github.com/MohitShridhar/RLBench/pull/1}.


\input{src/tab_gnfactor}
\noindent \textbf{Results on the GNFactor setup} 
We show quantitative results in Table~\ref{tab:gnfactor}. We train Act3D on this setup using its publicly available code. 
%\footnote{https://github.com/zhouxian/act3d-chained-diffuser}. 
\model{} outperforms both GNFactor and Act3D by a significant margin, achieving absolute performance gains of $+46.4\%$ and $+13.1\%$ respectively. Notably, \model{} and Act3D utilize similar 3D scene representations—sparse 3D feature tokens—while GNFactor featurizes a scene with 3D voxels and learns to reconstruct them. Even with a single camera view, both Act3D and \model{} outperform GNFactor significantly. This  suggests that the choice of 3D scene representation is a more crucial factor than the completion of 3D scenes in developing efficient 3D manipulation policies.


\input{src/tab_ablation}
\noindent \textbf{Ablations}
We ablate %design choices of \model{}, specifically 
the use of 3D scene representations and the use of relative attentions  in the PerAct experimental setup in Table \ref{tab:ablation}.  
%We use the PerAct experimental setup. 
We draw the following conclusions: 
\textbf{1.} \modellong{} largely outperforms its 2D counterpart, 2D Diffuser Actor, underlining the importance of 3D scene representations. 
\textbf{2.} \modellong{} with absolute 3D attentions (3D Diffuser Actor w/o Rel. Attn.) is much worse than \modellong{} with relative 3D attentions. This shows that translation equivariance through relative attentions is very important for generalization. Notably, this baseline already outperforms all prior arts in Table~\ref{tab:peract}, proving the effectiveness of marrying 3D representations and diffusion policies.


\input{src/tab_calvin}
\subsection{Evaluation on CALVIN} 
%\noindent \textbf{Setup}
The CALVIN benchmark  is build on top of the PyBullet~\cite{coumans2016pybullet} simulator and involves a Franka Panda Robot arm that manipulates the scene. CALVIN consists of 34 tasks\footnote{The definition of ``task" varies between different benchmarks: CALVIN considers the manipulation of variations (e.g., same objects with different colors) as different tasks, whereas, RLBench considers those the same task.} and 4 different environments (A, B, C and D). All environments are equipped with a desk, a sliding door, a drawer, a button that turns on/off an LED, a switch that controls a lightbulb and three different colored blocks (red, blue and pink).  These environments differ from each other in the texture of the desk and positions of the objects.  CALVIN provides 24 hours of tele-operated unstructured play data, 35\% of which are annotated with language descriptions.

We train \modellong{}  on the subset of play data annotated with language descriptions on the environments A, B and C and    evaluate it on 1000 unique instruction chains on environment D, following prior works ~\cite{li2023vision,wu2023unleashing}.  Each instruction chain includes five language instructions that need to be executed sequentially. We devise an algorithm (Appendix, Section~\ref{sec:heuristics_calvin}) to extract keyposes on CALVIN, since prior works do not use keyposes on this benchmark. We train our \model{} to predict both the end-effector pose for each keypose and the corresponding trajectory to reach the predicted pose, instead of using a motion planner. 
Prior works~\cite{mees2022hulc,black2023zero,li2023vision} predict a maximum of 360 actions to complete each instructional task, while, on average, it takes only 60 actions to complete each task using ground-truth trajectories.  
%In other words, models are allowed to explore the environment six times more than necessary. 
Our model predicts both keyposes and corresponding trajectories, and, on average, it takes 10 keyposes of each demonstration to complete an instructional task. We thus allow our model to predict a maximum of 60 keyposes for each task. For reference, we also allow our model to predict 360 times and show the influence of this hyperparameter in the Appendix (Section~\ref{sec:curve_calvin}).


\noindent \textbf{Baselines.} 
We consider the following baselines:
\begin{enumerate}
    \item MCIL~\cite{lynch2020language}, a multi-modal goal-conditioned 2D policy that maps three types of goals--goal images, language instructions and task labels--to a shared latent feature space, and conditions on such latent goals to predict actions.

    \item HULC~\cite{mees2022hulc}, a 2D policy that uses a variational autoencoder to sample a latent plan based on the current observation and task description, then conditions on this latent to predict actions.

    \item RT-1~\cite{brohan2022rt}, a 2D transformer-based policy that encodes the image and language into a sequence of tokens and employs a Transformer-based architecture that contextualizes these tokens and predicts the arm movement or terminates the episode.

    \item RoboFlamingo~\cite{li2023vision}, a 2D policy that adapts existing vision-language models, which are pre-trained for solving vision and language tasks, to robot control. It uses frozen vision and language foundational models and learns a cross-attention between language and visual features, as well as a recurrent policy that predicts the low-level actions conditioned on the language latents.

    \item SuSIE~\cite{black2023zero}, a 2D policy that deploys an large-scale pre-trained image generative model \cite{brooks2023instructpix2pix} to synthesize visual subgoals based on the current observation and language instruction. Actions are then predicted by a low-level goal-conditioned 2D diffusion policy that models inverse dynamics between the current observation and the predicted subgoal image.

    \item GR-1~\cite{wu2023unleashing}, a 2D policy that first pre-trains an autoregressive Transformer on next frame prediction, using a large-scale video corpus without action annotations. Each video frame is encoded into an 1d vector by average-pooling its visual features. Then, the same architecture is fine-tuned in-domain to predict both actions and future observations.

    \rebut{
    \item ChainedDiffuser~\cite{xian2023chaineddiffuser}, a combination of Act3D~\cite{gervet2023act3d} that predicts end-effector poses at key frames and a 3D trajectory predictor that generates intermediate trajectories to reach target end-effector poses.
    }
\end{enumerate}
We report results for HULC, RoboFlamingo, SuSIE and GR-1 from the respective papers. Results from MCIL are borrowed from \cite{mees2022hulc}. Results from RT-1 are copied from \cite{wu2023unleashing}.  \rebut{We evaluate ChainedDiffuser and \model{} with the final checkpoints across 3 seeds.  We report both the mean and standard deviation of evaluation results.}


\noindent \textbf{Evaluation metrics} 
Following previous works \cite{mees2022hulc,wu2023unleashing}, we report the success rate and the average number of completed sequential tasks.


\noindent \textbf{Results} 
We present our results in Table~\ref{tab:calvin}. \model{} achieves competitive results compared to the state-of-the-art models.  In comparison to GR-1, our model achieves absolute performance gains of \rebut{$+6.8\%$, $+9.1\%$, $+6.6\%$, $3.6\%$ and $+1.1\%$} for completing the 5 tasks in the instruction chain.  On average, \model{} complete \rebut{$3.35$} tasks in a row, setting a new state of the art. \rebut{In stark contrast, since Act3D fails to predict end-effector keyposes precisely, ChainedDiffuser does not work well on this benchmark, completing only $0.84$ tasks in a row.}. Note that GR-1's contribution is large-scale pre-training on videos, which is a scheme orthogonal to our contribution. Lastly, allowing our model to predict more times increases the performance significantly.
For this performance, we found stronger conditioning on the language instructions to be important, as we explain in our appendix (Figure~\ref{fig:detailed_diagram}b).


\input{src/tab_real}
\subsection{Evaluation in the real world}
We validate  \model{} in learning manipulation tasks from real-world demonstrations.  We use a Franka Emika robot and capture visual observations with a Azure Kinect RGB-D sensor at a front view.  Images are originally captured at $1280 \times 720$ resolution and downsampled to a resolution of $256 \times 256$.  Camera extrinsics are calibrated w.r.t the robot base.  We use 12 tasks: 1) {\it close a box}, 2) {\it put ducks in bowls}, 3) {\it insert a peg vertically into the hole}, 4) {\it insert a peg horizontally into the torus}, 5) {\it put a computer mouse on the pad}, %6) {\it rotate and open the bottle cap}, 
6) {\it open the pen}, 7) {\it press the stapler}, 8) {\it put grapes in the bowl}, %10) {\it align the screwdriver parallel to tools}, 
9) {\it sort the rectangle}, 10) {\it stack blocks with the same shape}, 11) {\it stack cups} and 12) {\it put block in a triangle on the plate}. Details on the task definitions and success criteria are included in the Appendix (Section~\ref{sec:real_world_tasks}).

We collect 15 demonstrations per task where we record the keyposes, most of which naturally contain noise and multiple modes of human behavior. For example, we pick one of two ducks to put in the bowl, we insert the peg into one of two holes and we put one of three grapes in the bowl, as shown in Figure \ref{fig:real}.
\model{} conditions on language descriptions and is trained to predict the next end-effector keypose. During inference, we utilize the BiRRT~\cite{kuffner2000rrt} planner provided by the MoveIt! ROS package \cite{coleman2014reducing} to reach the predicted poses. We evaluate 10 episodes for each task and report the success rate. 

We show quantitative results in Table~\ref{tab:real} and video results on our project webpage.


\subsection{Run time}
We measure the latency of our \model{} on CALVIN in simulation, using an NVIDIA GeForce 2080 Ti graphic card.  The wall-clock time of \model{} is 600 ms.   Notably, our model predicts end-effector keyposes sparsely, resulting in better efficiency than methods that predict actions densely at each time step. On CALVIN, on average, it takes 10 keyposes / 60 actions to complete each task using ground-truth trajectories.  Our \model{} can thus perform manipulation efficiently.


\subsection{Limitations}
\label{subsec:limitation}
Our framework currently has the following limitations: 
{\bf 1.} Our model conditions on 3D scene representations, which require camera calibration and depth information. 
{\bf 2.} All tasks in RLBench and CALVIN are quasi-static. Extending our method to dynamic tasks and velocity control is a direct avenue of future work.


==> rss_tex/rebuttal_final.tex <==

\newcommand{\sofn}[1]{{\color{cyan}SoFn}}
\newcommand{\rttc}[1]{{\color{purple}rTTc}}
\newcommand{\gyzr}[1]{{\color{blue}GyZr}}

% \input{src/fig_method_comparison}
\noindent \textbf{More clear comparison of 3D Diffuser Actor against Act3D and ChainedDiffuser.}
We present an overview comparison to Act3D~\cite{gervet2023act3d}, PerAct~\cite{shridhar2023perceiver} and Diffusion Policy~\cite{chi2023diffusion} in Figure~\ref{fig:compare} of the main paper.  We compare to Act3D and ChainedDiffuser in more detail in the following paragraphs.

\noindent \color{cyan} \textbf{3D Diffuser Actor vs. Act3D.} \color{black}
\textbf{\model{} is a diffusion model, iteratively denoising end-effector poses, while Act3D is a deterministic model, sampling and scoring 3D points in a coarse-to-fine manner to predict 3D locations, and regressing 3D orientations.} We include Figure~\ref{fig:compare} in the main paper and Figures \ref{fig:detailed_diagram} and \ref{fig:act3d_detailed_diagram} in the Appendix to show the differences between the models. %Figure~\ref{fig:detailed_diagram} in the Appendix for an illustration of our denoising 3D transformer model. 

\noindent Both Act3D and \model{} are methods that learn from demonstrations to predict 3D keyposes---\model{} also predicts 3D keypose trajectories---of the robot's end-effector, conditioned on multi-view RGB-D images and a language instruction.  
%Specifically, Act3D is a method that learns from demonstrations to predict 3D keyposes of the robot's end-effector, conditioned on multiview RGB-D images and a language instruction. 
Act3D predicts a variable spatial resolution 3D action map to represent the predicted 3D location of the end-effector (we say this in our related work: ``Act3D \cite{gervet2023act3d} foregoes 3D scene voxelization altogether; it instead computes a 3D action map of variable spatial resolution by sampling 3D points in the empty workspace and featurizing them using cross-attentions to the 3D physical points."). The action map is predicted by classifying different X,Y, Z locations, which helps translation-equivariance in prediction of the 3D location. The 3D end-effector orientation is regressed. 
%Main contribution: 
3D Diffuser Actor %is a method that learns to predict 3D keyposes as well as 3D keypose trajectories of the robot's end-effector conditioned on multiview RGB-D images and a language instruction using learning from demonstrations. \textbf{Main contribution: It
foregoes predicting 3D action maps altogether. It  %uses diffusion objectives to %handle multimodality in both 3D location and orientation prediction. } 
 %In spite of using a  scene encoder similar to Act3D, 
 %\model{} 
 considers action prediction as a denoising process conditioned on  images and language instructions, instead of a point classification problem.  
 


 
%\model{} represents the current estimate of the end-effector future pose trajectory as 3D tokens, that attend to scene 3D feature cloud and language tokens, and outputs the noise in the 3D translation and rotation.  It uses relative 3D attentions  among action tokens and the scene feature cloud.  At test time, \model{} initializes an estimate of end-effector poses from pure noise, and iteratively  denoises them to predict the final 3D keypose or keypose trajectories. 


\noindent \color{cyan} \textbf{3D relative attentions in \model{} vs. Act3D.} \color{black}
 %\textbf{Details of Act3D:} 
 Both Act3D and \model{} instantiate a scene 3D feature cloud by featurizing multiview RGB images and lifting the patch features to 3D using sensed depth. They also encode the language instruction using CLIP's language encoder. Act3D then samples 3D points (they call them ghost points) on a 3D grid.  It  contextualizes language tokens, scene tokens and sampled ghost point tokens using 3D relative attentions. %point them by cross-attending to the scene 3D feature cloud. 
 %A learnable query  cross-attends to the scene feature cloud and it is used to score all 3D ghost points and predict a 3D action map in this way, as well as regress the 3D rotation of the end-effector.} 
 %This process is repeated 3 times, each time with a refined 3D ghost point sampling and more fine-grained visual features to improve map resolution. At the end, 
 %The query features are also used to regress to a 3D rotation of the end-effector. % See Figure~\ref{fig:act3d_detailed_diagram} in the Appendix for the detailed diagram of Act3D.
 %\model{} follows a similar encoding process. 
 %\textbf{Implementation details of \model:}  
 %3D Diffuser Actor casts 3D keypose prediction as a denoising process conditioned on multiview images and language instructions. 
 %\model featurizes the RGB multiview images using a 2D pretrained backbone (CLIP) and lifts the 2D feature maps into a 3D featured cloud. It then embeds the language instruction using a CLIP language encoder (similar to Act3D and CLIPort among others). 
 3D Diffuser Actor uses a neural network that takes as input scene tokens, language tokens, a current estimate of the end effector’s 3D rotation and 3D translation and the index of the denoising iteration of diffusion, and outputs the noise in the 3D translation and rotation of the end effector. %, it uses FiLM layers to input the denoising iteration and instantiates a set of 3D tokens for the current end-effector trajectory estimate. 
 This denoising network also uses relative 3D  attentions to fuse all this information (we cite Act3D as an inspiration for that). 3D Diffuser's Actor 3D relative transformer is very different from Act3D's: 3D Diffuser Actor does not use 3D ghost point grids or coarse-to-fine featurizations. %The noisy keypose token, visual tokens and proprioception tokens are fed to a 3D relative self-attention layer that also updates the scene feature tokens. 
 \textbf{So, both models are in 3D and use relative attentions but on very different set of tokens.}
 Moreover, the scene tokens are updated in our case, while being frozen in Act3D. Figures \ref{fig:detailed_diagram} and \ref{fig:act3d_detailed_diagram} in the Appendix illustrate these technical differences.

\begin{comment}

The models of Act3D and 3D Diffuser Actor are thus different in that:
\begin{itemize}
    \item 

    \item They have different inputs and outputs. One maps x to y directly through coarse to fine 3D point sampling for 3D location and regression for 3D rotation, the other is a denoising diffusion model that takes x and the current y estimate (3D location and 3D rotation) and iteration index and predicts the noise in the current estimate.

   \item 3D Diffuser Actor does not build a 3D map (a map of 3D locations where each one is scored whether it contains the next end-effector 3D keypose or not).
   
    \item There is no coarse-to-fine sampling or any form of point sampling in 3D Diffuser Actor.


    \item The 3D relative attentions differ as noted above: 1) the token sets over which these attentions are conducted are different as explained above, 2) one is a cross-attention and the other a self-attention.
\end{itemize}
\end{comment}


%The main contribution of Act3D is to (1) forego expensive 3D voxelization and (2) preserve equivariance to facilitate generalization in action prediction, by predicting a 3D point action map.  Act3D converts multiview posed RGB-D images into a 3D feature cloud, and encodes language instructions into language tokens.  To obtain a 3D point map, Act3D samples 3D ghost points on a 3D grid, initializes a query token for each sampled points, and features point tokens by cross-attending to the scene 3D feature cloud.  To predict action with the 3D point map, Act3D additionaly initializes a learnable query, that cross-attends to both the 3D feature cloud and language tokens, and scores each sampled point with the similarity of token features.  This process is repeated 3 times, each time with a refined 3D point sampling and more fine-grained visual features to improve map resolution.  At the end, a 3D rotation of the end-effector is regressed from the query features, and a 3D location of the end-effector is derived from the location of the point with the maximal activation.  Act3D is thus a deterministic policy.

%The main contribution of \model{} is to (1) forego building 3D point maps and (2) iteratively denoise end-effector poses to handle multimodality in action prediction.  In spite of using the similar scene encoder as Act3D, \model{} considers action prediction as a denoising process conditioned on multiview images and language instructions, instead of a point classification problem.  Our model represents current estimate of the end-effector poses as 3D tokens, that attend to scene 3D feature cloud and language tokens, and outputs the noise in the 3D translation and rotation of the end effector.  To preserve translation invariance, we apply relative attention using relative positions among pose tokens and the scene feature cloud.  \model{} initializes estimate of end-effector poses from pure noise, iterates the denoising process, and at the end, outputs the end-effector poses.

%In summary, \model{} differs from Act3D as the former is a diffusion model, iteratively denoising end-effector poses, and the latter is a deterministic model, sampling and scoring 3D points in a fine-to-coarse manner.

%\noindent 
\noindent \color{cyan} \textbf{\model{} vs. ChainedDiffuser.} \color{black}
\model{} is significantly different from ChainedDiffuser.  ChainedDiffuser is a method that combines Act3D and a trajectory diffusion model.  The end-effector poses at key frames are predicted deterministically by Act3D. A trajectory diffusion model \textbf{conditions on Act3D's predicted 3D keyposes} to denoise trajectories to link the current pose to the Act3D's predicted pose. The contribution of ChainedDiffuser is to get rid of sampling-based motion planners, as they fail in tasks that cannot be easily decomposed into straight-line trajectory segments, such as {\it opening doors} or {\it wiping the table}.  %It uses trajectory diffusion that conditions on the current and target end-effector poses to predict the intermediate trajectory.
In contrast, \textbf{\model{} is a single diffusion policy that predicts both end-effector poses at key frames and intermediate trajectory to reach end-effector keyposes.} 
%The contribution of \model{} is to propose a single diffusion framework for predicting both (1) end-effector poses at key frames, and (2) the intermediate trajectory to reach target poses.  Our model can thus handle multimodality of action prediction better than ChainedDiffuser. 

\noindent Per the reviewers' request,  we tested ChainedDiffuser on CALVIN as shown in Table~\ref{tab:calvin}, and \model{} greatly outperforms it. The reason is that Act3d predicts 3D end effector orientations in a deterministic way, which is very limiting in CALVIN that has very multimodal demonstrations.



%ChainedDiffuser is a method that takes as input 3D keyposes predicted by Act3D and predicts end-effector trajectories to link the current keypose to the predicted one. Main contribution: ChainedDiffuser proposes to get rid of sampling-based motion planners (like RRT) because they fail in tasks that cannot be easily decomposed into straight-line trajectory segments, such as opening doors or wiping the table, and instead uses trajectory diffusion that conditions on the current and predicted 3D end-effector keyposes to predict a 3D end-effector trajectory that links them.

%Details: ChainedDiffuser uses an architecture similar to Act3D to create a 3D feature cloud and takes as input the current trajectory estimate to predict scaled noise for translation trajectory and the final denoised rotation trajectory. It shows that in tasks that require continuous motion, Act3D keyposes in combination with this trajectory denoising from keypose to keypose, much outperforms Act3D+motion planners. ChainedDiffuser’s contribution is a learnt trajectory predictor that works alongside an off-the-shelf 3D keypose prediction method. ChainedDiffuser is complementary to our work: We can use keyposes predicted by 3D Diffuser Actor and link them with ChainedDiffuser’s trajectories instead of motion planners and achieve similar boosts in these tasks. Because the tasks in the PerAct benchmark that we consider do not require such continuous trajectories, motion planners work well, so we did not use a trajectory prediction model.%; ChainedDiffuser performs as well as Act3D there (no additional performance boost).

%The diffusion models of ChainedDiffuser and 3D Diffuser Actor are thus different in that: 1. ChainedDiffuser takes as input the to-reach 3D keypose while 3D Diffuser Actor tries to predict it. In that sense, 3D Diffuser Actor has a much much harder task to solve. \fixme{2. 3D Diffuser Actor denoises 3D keyposes and trajectories and ChainedDiffuser denoises 3D trajectories.} 3. The experiments in ChainedDiffuser concern single manipulation tasks while 3D Diffuser Actor shows multi-task results across the whole PerAct suite.

%The models of ChainedDiffuser and 3D Diffuser Actor are similar in that:

%Both build 3D feature clouds and use diffusion to predict their desired output, being the next 3D keypose for 3D Diffuser Actor and being a current to predicted 3D keypose trajectory for ChainedDiffuser.
%ChainedDiffuser can take as input the keyposes predicted by 3D Diffuser Actor and we explained above why we did not consider this.


\noindent \color{cyan}\textbf{Details on the 3D scene representation.} \color{black} 
We use a 3D scene encoder similar to \cite{gervet2023act3d,xian2023chaineddiffuser}, which extract 3D scene tokens from posed RGB-D images and gather tokens from multiple camera views into 3D feature cloud.  Our \model{} conditions on the 3D feature cloud and diffuses the trajectory of end-effectory poses. 
For each camera view $i$, we capture the RGB image $I_{i} \in \mathbb{R}^{H\times W\times 3}$ and the depth map $D_{i} \in \mathbb{R}^{H\times W}$, where $H, W$ denote the height and width in pixels. We obtain a 3D location map $P_i \in \mathbb{R}^{H\times W\times 3}$ by mapping each pixel location and depth value to a 3D location in the world frame, using the camera extrinsic/intrinsic parameters and the pinhole camera equation. We obtain scene features by encoding each image $I_i$ to a 2D feature map $F_i \in \mathbb{R}^{\frac{H}{s} \times \frac{W}{s} \times c}$, where $s$ denotes the downsampling ratio of the image encoder and $c$ is the channel dimension. To obtain the 3D scene tokens, we need to map each feature vector in $F_i$ to a 3D location.  We downsample $P_i$ to $P'_i \in \mathbb{R}^{\frac{H}{s} \times \frac{W}{s} \times 3}$ with 2D average pooling, where $P'_i(u, v)$ corresponds to the 3D location of feature vector $F_i(u, v)$ at patch $(u, v)$.  Lastly, we gather 3D scene tokens from multiple camera views into a 3D feature cloud, consisting of token features $\mathbf{F} = \{F_i(u, v) | \forall u, v\}_{i=1}^{N_C}$ and 3D location $\mathbf{P'} = \{P'_i(u,v) | \forall u, v\}_{i=1}^{N_C}$, where $u, v$ denote the row and column index of patch, $i$ is the camera index and $N_C$ is the total number of camera views.  We updated the main paper with this detailed description.


\noindent \color{cyan}\textbf{Details of 3D relative  transformer.} \color{black} 
We use a 3D relative transformer to diffuse a trajectory of end-effector poses $\mathbf{A} = \{\ac_j\}_{\forall j}$, where $\ac_j = \{\ac^{pos}_j, \ac^{rot}_j, \ac_j^{open}\}$ denotes the $j^{th}$ pose in the trajectory.  At each diffusion step $t$, we represent the estimate of $j^{th}$ pose $\ac_{j,t}$ as a 3D token in the transformer, which attends to 3D scene tokens, all pose estimates $\mathbf{A}_t = \{\ac_{j,t}\}_{\forall j}$, and language instruction tokens to denoise current estimate of the end-effector pose.

In particular, we map the position $\ac^{pos}_{j,t}$ and rotation $\ac^{rot}_{j,t}$ to a pose token with a MLP, where $\ac^{pos}_{j,t}$ corresponds to the 3D location of the pose token.  We apply cross-/self-attention among all scene tokens $\mathbf{F}$ and all pose tokens using their 3D locations $\mathbf{P'}$ and $\mathbf{A}_t^{pos} = \{\ac_{j,t}^{pos}\}_{\forall j}$.  To ensure translation invariance in the denoising transformer, we use the rotary positional embeddings~\cite{su2021roformer} to encode relative positional information in attention layers, inspired by recent work in visual correspondence \cite{Li2021LepardLP,Gkanatsios2023AnalogyFormingTF} and 3D manipulation \cite{gervet2023act3d,xian2023chaineddiffuser}.  The attention weight between query $q$ and key $k$ is written as: $e_{q, k} \propto \mathbf{x}_q^T \mathbf{M}(\mathbf{p}_q - \mathbf{p}_k) \mathbf{x}_k$, where $\mathbf{x}_q$ / $\mathbf{x}_k$ and $\mathbf{p}_q$ / $\mathbf{p}_k$ denote the features and 3D positions of the query / key, and $\mathbf{M}$ is a matrix function which depends only on the relative positions of the query and key.  We provide a more detailed formulation in Section~\ref{sec:attention} of the Appendix.

Lastly, we use separate MLPs to predict (1) the noise of position $\epsilon_\theta^{\mathrm{\small pos}}(o, l, c,\mathbf{A}_{\id}^{\mathrm{\small pos}}, \mathbf{A}_{\id}^{\mathrm{\small rot}},\id)$, (2) the noise of rotation $\epsilon_\theta^{\mathrm{\small rot}}(o, l, c, \mathbf{A}_{\id}^{\mathrm{\small pos}},\mathbf{A}_{\id}^{\mathrm{\small rot}},\id)$ and (3) the openess of the end-effector $f_\theta^{\mathrm{\small open}}(o,l,c,\mathbf{A}_{\id}^{\mathrm{\small pos}},\mathbf{A}_{\id}^{\mathrm{\small rot}},\id)$, from pose tokens.  Here, $o$ denotes the visual observations, $l$ the input language and $c$ the proprioception information. We provide a detailed diagram of our model in Fig.~\ref{fig:detailed_diagram} of the Appendix.

\noindent \color{cyan}\textbf{Robustness to noisy calibrations?} \color{black} 
\model{} is reasonably robust to noisy calibrations.  We evaluate our model on RLBench with the setup of GNFactor.  We perturb the depth information by adding Gaussian noise to the 3D location of each pixel.  Under mild ($\sigma=0.01$) and strong ($\sigma=0.03$) perturbations, \model{} retains $92\%$ and $64\%$ of the relative performance of that without noise.  Notably, our model has only been trained with perfect calibrations.  We can further enhance the robustness to noisy calibrations by impose corresponding augmentations during training.  We present our experimental results in Table~\ref{tab:noisy_depth} and Section~\ref{sec:noisy_depth} in the Appendix.

\noindent \color{cyan}\textbf{Failure modes?} \color{black} 
We discover two major failure modes of \model{}: (1) imprecise action prediction, and (2) confusion of language instruction.  In $50\%$ of the failure cases, it does not predict end-effector poses precisely and fails to satisfy the success condition.  In $38\%$ of the failure cases, it does not grasp the target object specified in the language instruction.  In $8\%$ of the failure cases, it fails on an intermediate task of a long-horizon task.  In the rest of the failure cases, the motion planner fails to find an optimal path to reach the predicted end-effector pose.  We present the analysis in Figure~\ref{fig:failure} and Section~\ref{sec:failure} in the Appendix.

==> src/fig_task.tex <==
\begin{figure*}
    % \centering
    % \vspace{-10pt}
    \begin{adjustbox}{center}
    \includegraphics[width=1.0\textwidth,keepaspectratio]{figs/tasks.pdf}
    \end{adjustbox}
    \caption{\textbf{Manipulation tasks in simulation and the real world.} We conduct experiments on 18 simulated tasks in RLBench \cite{james2020rlbench}  and 12 real-world tasks.  We show only 5 tasks for each setup. A thorough description of both our real-world tasks and the RLBench tasks is included in the Appendix (Sections~\ref{sec:real_world_tasks},\ref{sec:rlbench_tasks}).
    }
    \label{fig:tasks}
\end{figure*}

==> src/tab_act3d.tex <==
\begin{table*}[t]
    \centering
    \begin{adjustbox}{width=\textwidth}
    \tb{@{}l|c|c|c|c|c|c|c|c|c|c@{}}{1.0}{
    & Avg. & open & slide & sweep to & meat off & turn & put in & close & drag & stack \\
    & Success $\uparrow$ & drawer & block & dustpan & grill & tap & drawer & jar & stick & blocks \\
    \midrule
    HiveFormer~\cite{hiveformer} & 45 & 52 & 64 & 28 & \textbf{100} & 80 & 68 & 52 & 76 & 8\\
    PolarNet~\cite{Chen2023PolarNet3P} & 46 & 84 & 56 & 52 & \textbf{100} & 80 & 32 & 36 & 92 & 4\\
    Act3D~\cite{gervet2023act3d} & 65 & 93 & 93 & 92 & 94 & 94 & 90 & 92 & 92 & 12\\
    \model{} (ours) & \textbf{78} & \textbf{97} & 94 & \textbf{99} & 95 & \textbf{99} & \textbf{92} & \textbf{97} & 97 & \textbf{72} \\
    \midrule\midrule
    & screw & put in & place & put in & sort & push & insert & stack & place \\
    & bulb & safe & wine & cupboard & shape & buttons & peg & cups & cups & \\
    \midrule
    HiveFormer~\cite{hiveformer} & 8 & 76 & 80 & 32 & 8 & 84 & 0 & 0 & 0 &\\
    PolarNet~\cite{Chen2023PolarNet3P} & 44 & 84 & 40 & 12 & 12 & 96 & 4 & 8 & 0 & \\
    Act3D~\cite{gervet2023act3d} & 47 & 95 & 80 & 51 & 8 & 99 & 27 & 9 & 3 &\\
    \model{} (ours) & \textbf{89} & \textbf{100} & \textbf{95} & \textbf{69} & \textbf{13} & \textbf{100} & \textbf{32} & \textbf{55} & \textbf{16} &\\
    \bottomrule
    }
    \end{adjustbox}
    \caption{\textbf{Multi-Task performance on RLBench under Act3D setup.} We report success rates on 18 RLBench tasks of the same test split as Act3D~\cite{gervet2023act3d}.  We evaluate the final checkpoint over 1 random seeds with the same 3D object models and success conditions of RLBench~\cite{james2020rlbench} as Act3D.  Four camera views are used for all experiments.  We show the performance gain compared to other best performing baselines other than \model{}.  Our \model{} outperforms all prior arts among most tasks by a large margin.
    }
    \label{tab:act3d}
\end{table*}

% \begin{table*}[t]
%     \centering
%     \begin{adjustbox}{width=\textwidth}
%     \tb{@{}c|l|c|c|c|c|c|c|c|c|c|c@{}}{1.0}{
%     \multicolumn{2}{c|}{} & Avg. & Avg. & open & slide & sweep to & meat off & turn & put in & close & drag \\
%     \multicolumn{2}{c|}{} & Success $\uparrow$ & Rank $\downarrow$  & drawer & block & dustpan & grill & tap & drawer & jar & stick\\
%     \midrule
%     & HiveFormer~\cite{hiveformer} & 45 &  & 52 & 64 & 28 & \textbf{100} & 80 & 68 & 52 & 76\\
%     & PolarNet~\cite{Chen2023PolarNet3P} & 46 & & 84 & 56 & 52 & \textbf{100} & 80 & 32 & 36 & 92\\
%     & Act3D~\cite{gervet2023act3d} & 65 & 3.4 & 93 & 93 & 92 & 94 & 94 & 90 & 92 & 92\\
%     \midrule
%     \multirow{4}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1cm}{\centering Ablations}}}  & 2D Diffuser Actor & 44 & 4.9 & 68 & 65 & 90 & 75 & 72 & 55 & 94 & 79 \\
%     & 3D Diffuser Actor w/o Rel. Attn. & 68 & 2.6 & 96 & \textbf{99} & 87 & 98 & 97 & 91 & 94 & 98 \\
%     & 3D Regressor Actor & & & & & & & & & & \\
%     & \model{} (ours) & 
%     \textbf{78} (\bluebf{+13}) & \textbf{1.3}  & \textbf{97} (\bluebf{+4}) & 94 (\bluebf{+1}) & \textbf{99} (\bluebf{+7}) & 95 (\bluebf{+1}) & \textbf{99} (\bluebf{+3}) & \textbf{92} (\bluebf{+2}) & \textbf{97} (\bluebf{+5}) & 97 (\bluebf{+5})\\
%     \midrule
%     \multicolumn{2}{c|}{} & stack & screw & put in & place & put in & sort & push & insert & stack & place \\
%     \multicolumn{2}{c|}{} & blocks  & bulb & safe & wine & cupboard & shape & buttons & peg & cups & cups \\
%     \midrule
%     & HiveFormer~\cite{hiveformer} & 8 & 8 & 76 & 80 & 32 & 8 & 84 & 0 & 0 & 0\\
%     & PolarNet~\cite{Chen2023PolarNet3P} & 4 & 44 & 84 & 40 & 12 & 12 & 96 & 4 & 8 & 0\\
%     & Act3D~\cite{gervet2023act3d} & 12 & 47 & 95 & 80 & 51 & 8 & 99 & 27 & 9 & 3\\
%     \midrule
%     \multirow{4}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1cm}{\centering Ablations}}} & 2D Diffuser Actor & 1 & 48 & 57 & 68 & 3 & 0 & 9 & 6 & 0 & 0 \\
%     & 3D Diffuser Actor w/o Rel. Attn. & 35 & 48 & 97 & 94 & 64 & 7 & 98 & 6 & 12 & 0 \\
%     & 3D Regressor Actor & & & & & & & & & & \\
%     & \model{} (ours) & \textbf{72} (\bluebf{+60}) & \textbf{89} (\bluebf{+42}) & \textbf{100} (\bluebf{+5}) & \textbf{95} (\bluebf{+15}) & \textbf{69} (\bluebf{+18}) & \textbf{13} (\bluebf{+5}) & \textbf{100} (\bluebf{+1}) & \textbf{32} (\bluebf{+5}) & \textbf{55} (\bluebf{+46}) & \textbf{16} (\bluebf{+13})\\
%     \bottomrule
%     }
%     \end{adjustbox}
%     \caption{\textbf{Multi-Task Performance on RLBench under Act3D setup.} We report success rates on 18 RLBench tasks of the same test split as Act3D~\cite{gervet2023act3d}.  We test the final checkpoint over 1 random seed with the same RLBench~\cite{james2020rlbench} as Act3D.  Four camera views are used for all experiments.  We show the performance {\color{blue} gain} compared to Act3D.  Our \model{} outperforms Act3D and ablative baselines among most tasks.}
%     \label{tab:act3d}
% \end{table*}


% \begin{table*}[t]
%     \centering
%     \begin{adjustbox}{width=\textwidth}
%     \tb{@{}c|l|c|c|c|c|c|c|c|c|c|c@{}}{1.0}{
%     \multicolumn{2}{c|}{} & Avg. & Avg. & open & slide & sweep to & meat off & turn & put in & close & drag \\
%     \multicolumn{2}{c|}{} & Success $\uparrow$ & Rank $\downarrow$  & drawer & block & dustpan & grill & tap & drawer & jar & stick\\
%     \midrule
%     & PerAct~\cite{shridhar2023perceiver} & 49 & 4.5 & 88 & 74 & 52 & 70 & 88 & 51 & 55 & 90\\
%     & RVT~\cite{goyal2023rvt} & 63 & 3.5 & 71 & 82 & 72 & 88 & 94 & 88 & 52 & 99\\
%     & Act3D~\cite{gervet2023act3d} & 65 & 3.4 & 93 & 93 & 92 & 94 & 94 & 90 & 92 & 92\\
%     \midrule
%     \multirow{3}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1cm}{\centering Ablations}}}  & 2D Diffuser Actor & 44 & 5.9 & 68 & 65 & 90 & 75 & 72 & 55 & 94 & 79 \\
%     & 3D Diffuser Actor w/o Rel. Attn. & 68 & 2.6 & 96 & \textbf{99} & 87 & 98 & 97 & 91 & 94 & 98 \\
%     & \model{} (ours) & 
%     \textbf{78} (\bluebf{+13}) & \textbf{1.3}  & \textbf{97} (\bluebf{+4}) & \textbf{94} (\bluebf{+1}) & \textbf{99} (\bluebf{+7}) & 95 (\bluebf{+1}) & \textbf{99} (\bluebf{+3}) & \textbf{92} (\bluebf{+2}) & 97 (\bluebf{+5}) & 97 (\bluebf{+5})\\
%     \midrule
%     \multicolumn{2}{c|}{} & stack & screw & put in & place & put in & sort & push & insert & stack & place \\
%     \multicolumn{2}{c|}{} & blocks  & bulb & safe & wine & cupboard & shape & buttons & peg & cups & cups \\
%     \midrule
%     & PerAct~\cite{shridhar2023perceiver} & 26 & 18 & 86 & 45 & 28 & 17 & 93 & 6 & 2 & 2\\
%     & RVT~\cite{goyal2023rvt} & 29 & 48 & 91 & 91 & 50 & 36 & 100 & 11 & 26 & 4\\
%     & Act3D~\cite{gervet2023act3d} & 12 & 47 & 95 & 80 & 51 & 8 & 99 & 27 & 9 & 3\\
%     \midrule
%     \multirow{3}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1cm}{\centering Ablations}}} & 2D Diffuser Actor & 1 & 48 & 57 & 68 & 3 & 0 & 9 & 6 & 0 & 0 \\
%     & 3D Diffuser Actor w/o Rel. Attn. & 35 & 48 & 97 & 94 & 64 & 7 & 98 & 6 & 12 & 0 \\
%     & \model{} (ours) & \textbf{72} (\bluebf{+60}) & \textbf{89} (\bluebf{+42}) & \textbf{100} (\bluebf{+5}) & \textbf{95} (\bluebf{+15}) & \textbf{69} (\bluebf{+18}) & \textbf{13} (\bluebf{+5}) & \textbf{100} (\bluebf{+1}) & \textbf{32} (\bluebf{+5}) & \textbf{55} (\bluebf{+46}) & \textbf{16} (\bluebf{+13})\\
%     \bottomrule
%     }
%     \end{adjustbox}
%     \caption{\textbf{Multi-Task Performance on RLBench under Act3D setup.} We report success rates on 18 RLBench tasks of the same test split as Act3D~\cite{gervet2023act3d}.  We test the final checkpoint over 1 random seed with the same RLBench~\cite{james2020rlbench} as Act3D.  Four camera views are used for all experiments.  We show the performance {\color{blue} gain} and {\color{red} loss} compared to Act3D.  Our \model{} outperforms Act3D and ablative baselines among most tasks.}
%     \label{tab:peract}
% \end{table*}

==> src/tab_calvin_sota.tex <==
\begin{table*}[t]
    \centering
    \begin{adjustbox}{width=0.9\textwidth}
    \tb{@{}l|c|ccccccc@{}}{2.0}{
    & Train & \multicolumn{6}{c}{Task completed in a row} \\
    & episodes & 1 & 2 & 3 & 4 & 5 & Avg. Len \\
    \midrule
    MCIL~\cite{lynch2020language} & All & 30.4 & 1.3 & 0.2 & 0.0 & 0.0 & 0.31\\
    HULC~\cite{mees2022hulc} & All & 41.8 & 16.5 & 5.7 & 1.9 & 1.1 & 0.67 \\
    RT-1~\cite{brohan2022rt} & Lang & 53.3 & 22.2 & 9.4 & 3.8 & 1.3 & 0.90 \\
    RoboFlamingo~\cite{li2023vision} & Lang & 82.4 & 61.9 & 46.6 & 33.1 & 23.5 & 2.48 \\
    SuSIE~\cite{black2023zero} & All & 87.0 & 69.0 & 49.0 & 38.0 & 26.0 & 2.69 \\
    GR-1~\cite{wu2023unleashing} & Lang & 85.4 & 71.2 & 59.6 & 49.7 & 40.1 & 3.06 \\
    \model{} (ours, 60 keyposes) & Lang & \textbf{92.2} & \textbf{78.7} & \textbf{63.9} & \textbf{51.2} & \textbf{41.2} & \textbf{3.27} \\
    \bottomrule
    }
    \end{adjustbox}
    \caption{\textbf{Zero-shot long-horizon performance on CALVIN.}  We show our new results on CALVIN, where we enhance the conditioning of language instructions by adding more cross-attention layers from 3D scene tokens and current pose estimate to the language encodings.  We report success rates and average length of completed task sequences.  All models are trained on play trajectories on environments A, B, C, and tested on 1000 unique instruction chains on environment D.  MCIL, HULC and SuSIE are trained with all play trajectories in the training scenes, whereas, RT-1, RoboFlamingo, GR-1 and our \model{} are trained with the subset of play data annotated with language descriptions.  Our \model{} sets new state-of-the-art, outperforming all other prior arts by a large margin.
    }
    \label{tab:sota_calvin}
\end{table*}


==> src/tab_runtime.tex <==
\begin{wraptable}{r}{5.5cm}
    \begin{adjustbox}{width=\linewidth}
    \centering
    \tb{@{}l|c|c|c@{}}{0.6}{
     & runtime (ms) & \# of actions \\
    \midrule
    \model{} & 600 & 20 \\
    ChainedDiffuser & 1170 & 20 \\
    3D Diffusion Policy & 581 & 3 \\
    \bottomrule
    }
    \end{adjustbox}
    \caption{\textbf{Control frequency on CALVIN. \todo{recompute these numbers}}}
    \label{tab:runtime}
\end{wraptable}


==> src/tab_single.tex <==
\begin{figure}[H]
    %\centering
     \begin{adjustbox}{center}
     \includegraphics[width=\linewidth]{figs/hiveformer_results.png}
     \end{adjustbox}    
    \caption{\textbf{Single-task performance.} On 74 tasks, spanning nine different categories, \model{} outperforms prior state-of-the-art models InstructRL and Act3D.}
    \label{fig:hiveformer_results}
\end{figure}
